Counter-example guided Imitation Learning of Feedback Controllers from Temporal Logic Specifications

We present a novel method for imitation learning for control requirements expressed using Signal Temporal Logic (STL). More concretely we focus on the problem of training a neural network to imitate a complex controller. The learning process is guided by efficient data aggregation based on counter-examples and a coverage measure. Moreover, we introduce a method to evaluate the performance of the learned controller via parameterization and parameter estimation of the STL requirements. We demonstrate our approach with a flying robot case study.

==> figures/flying_robot.tex <==
\begin{figure}
    \centering
    \begin{tikzpicture}[rotate=15,transform shape]
        % robot body
        \draw (-1.2,-0.8) rectangle (1.2,0.8);
        %
        % thrusters
        \draw (-0.5,1.2) rectangle (0.5,1.6);
        \draw (-0.1,0.8) rectangle (0.1,1.2);
        \begin{scope}[yscale = -1]
            \draw (-0.5,1.2) rectangle (0.5,1.6);
            \draw (-0.1,0.8) rectangle (0.1,1.2);
        \end{scope}
        %
        % thrusts
        \draw (0.5,1.3) -- (0.8,1.3);
        \draw (0.5,1.4) -- (0.8,1.4);
        \draw (0.5,1.5) -- (0.8,1.5);
        \node (u1) at (1,1.4) {$u_1$};
        \begin{scope}[yscale = -1]
            \draw (0.5,1.3) -- (0.8,1.3);
            \draw (0.5,1.4) -- (0.8,1.4);
            \draw (0.5,1.5) -- (0.8,1.5);
        \end{scope}
        \node (u2) at (1,-1.4) {$u_2$};
        %
        % \draw (0,0) -- (-1,-1);
        %
        % representing theta
        \draw[->] (0,0) -- (2.3,0);
        \draw[dashed,rotate around = {-15:(0,0)}] (0,0) -- (2.3,0);
        \draw (1.5,0) arc (0:-15:1.5);
        \node (theta) at (1.7,-0.225) {$\theta$};
        %
        % legs?
        \draw (-1.2,0.6) -- (-2,0.5);
        \draw (-1.2,-0.6) -- (-2,-1);
        \draw (-2,0.5) -- (-1.6,0.3);
        \draw (-2,-1) -- (-2,-0.5);
    \end{tikzpicture}
    \caption{Flying Robot with two thrusters \cite{flying_robot_mathworks}}
    \label{fig:flying_robot} 
\end{figure}

==> figures/mining_fig.tex <==
\begin{figure}
    \centering
    
  \begin{tikzpicture}[>=stealth',scale=.5, transform shape]

    % \path (-4,0) -- (12,-9);

    %% Styles
\tikzstyle{smalltext}=[font=\fontsize{10}{10}\selectfont]
\tikzstyle{block}=[draw,fill=white, rectangle,minimum height=2em,text width=8em, smalltext, text centered]
\tikzstyle{tool}=[draw,rectangle,rounded corners,minimum height=3em,minimum width=10mm,text
width=25mm, text centered, smalltext, top color=white, bottom color=blue!30, draw=blue!50!black!100, drop
shadow]
\tikzstyle{file}=[tape,fill=red!10,tape bend top=none,draw=gray, smalltext, text centered]

%% Nodes
\node[coordinate] (input) {};
\node[coordinate] [left of=input, node distance=5mm] (inputCor) {};
\node[right of=input, draw,fill=white,circle,node distance=7mm,inner sep=2pt] (sum) {$+$};
\node[coordinate,below of=sum,node distance=10mm] (b) {};
\node[block,node distance=20mm,right of=sum, text width=20mm] (c) {Controller};
\node[block,node distance=38mm,right of=c, text width=28mm] (p) {Plant Model};

\draw[->] (sum) -- node [above] {$e$} (c);
\draw[->] (c) -- node [above] {$u$} (p);
\draw[->] (p) |- node [right,pos=0.3] {$y$} (b) -- (sum);
\draw[->] (inputCor) -- (sum);

\begin{pgfonlayer}{background}
    \node[file,
          fit=(sum) (c) (p) (b) (input),inner sep=7pt]
          (simulink) {};
\end{pgfonlayer}

\coordinate (simLower) at ($(simulink.west) + (0mm,-5mm)$);
\coordinate (simleft) at ($(simulink.west) + (41.5mm,-0.5mm)$);
\coordinate (simright) at ($(simulink.east) + (0mm,-5mm)$);
   
\node[coordinate,below of=simulink,xshift=0.6cm ,node distance=25mm] (mid2) {};
\node[coordinate,left of=mid2,node distance=50mm] (mid) {};

% node param synth
\node[tool,below of=mid,node distance=20mm] (breach) {ParamSynth};

% coordinates
\coordinate (breachNorth1) at ($(breach.north) - (2.5mm,0)$);
\coordinate (breachNorth2) at ($(breach.north) + (13mm,0)$);
\node [coordinate,above of=breach,node distance=20mm] (mid1) {};

% node simulation trace
\node [file,left of=mid1,node distance=2.5mm,text width=20mm] (traces) {Simulation Traces};

% node candidate specification
\node [file,right of=breach,node distance=45mm,text width=25mm] (candidate) {Candidate Specification};

% node counter example traces 
\node [file,above of=candidate,node distance=20mm,text width=30mm] (counterexample) {Counterexample Traces};

% node falsify
\node [tool,right of=candidate,node distance=45mm] (staliro) {Falsif};

% coordinates
\coordinate (staliroNorth2) at ($(staliro.north) + (1.5mm,0)$);

% node template
\node [rectangle,fill=white,text width=54mm,draw,node distance=25mm,below of=breach,smalltext] (template)
    {$\ev_{[0,\tPara_1]}(\mathtt{x_1}< \sPara_1 \wedge \alw_{[0,\tPara_2]}(\mathtt{x_2}>\sPara_2))$};

\begin{pgfonlayer}{background}
    \node [file,inner sep=7pt,fit=(template),label=below:{\small Template Specification}] (template) {};
\end{pgfonlayer}
% node assignement

\node [rectangle,draw, below right = 5mm and -5mm  of breach, fill=green ] {  $\tau_1 \leftarrow .7$, $\pi_1 \leftarrow 2$, $ \pi_2 \leftarrow 3 $  } ;

% node inferred
\uncover<8->{\node [rectangle,fill=white,text width=54mm,draw,node distance=25mm,below of=staliro,smalltext] (inferred)
    {$\ev_{[0,1.1]}(\mathtt{x_1}< 3.7 \wedge \alw_{[0,5]}(\mathtt{x_2}>0.1))$};

\begin{pgfonlayer}{background}
  \node [file,inner sep=7pt,fit=(inferred),label=below:{\small Inferred Specification}] (inferred) {};
\end{pgfonlayer}
}

\draw[->] (simLower) -| node [pos=.5, left] {init} (traces);

\draw[<->] (simright) -| (staliroNorth2);
\draw[->] (traces) -- (breachNorth1);
\draw[->] (template) -- (breach);
\draw[->] (breach) -- (candidate);
\draw[->] (candidate) -- (staliro);
\draw[->] (staliro) |- node[below,pos=0.75,text width=10mm,smalltext] {Counter-example Found} (counterexample);
\draw[->] (counterexample.west) -- (traces);
\draw[->] (staliro) -- node[left,smalltext ] {No Counterexample} (inferred);

\end{tikzpicture}
    \caption{Overview of the approach.}
    \label{fig:approach}
\end{figure}



==> iccps2023_version/algorithm.tex <==
\section{Controller Learning Methodology}
\label{sec-methodology}

In this section, we present our methodology for learning a feedback controller through counterexample guided retraining.

\subsection{Neural Net Structure and Training} Intuitively, the NN controller is trained based on the desired closed-loop behaviours we want it to learn. Let $\traj = (r(\cdot), x(\cdot), u(\cdot), y(\cdot), \dis(\cdot))$ be a desired closed-loop behaviour, from which we extract the data of the form \begin{equation}\label{eq:dataextraction}
\data_{\traj} = \bigl\{ (r_k, y_k, u_k, \dis_k) \bigm| k < K \bigr\}
\end{equation}
where $r_k$, $y_k$, $u_k$, and $\dis_k$ are respectively the reference value, output value, control value, and the disturbance at time $t_k$; $K$ is the discrete time horizon (that is, the number of sampled time points). When many desired behaviours are considered, the data set $\dataset$ is the union of all $\data_{\traj}$. We generate a neural net $\neuralnet$ to match the data set $\dataset$. The structure of the NN should capture the input-output relationship of the controller in \eqref{eq:controller}. We add past values to represent the memory needed to compute the output at each discrete step. The input of the neural net is
$(r_k, r_{k-1},\ldots, r_{k-n_r}, \overline{y}_k, \overline{y}_{k-1}, \ldots, \overline{y}_{k-n_y}, \overline{u}_{k-1}, \ldots$, $\overline{u}_{k-n_u}$, $\dis_k, \dis_{k-1},\ldots, \dis_{k-n_{\dis}})$ where $n_r$,$n_y$, $n_u$, $n_{\dis}$ represent the number of previous values (memory) of $r_k$, $y_k$, $u_k$, and $\dis_k$ respectively that are needed for training, and the output is $\overline{u}_k$.  
To train the NN, we use a loss function defined via the Mean Square Error (MSE): ${\frac{1}{N}\sum_{k=1}^N (u_k-\overline{u}_k)^2}$, where $u$ is the output of the nominal controller and $\overline{u}$ is the output of the NN. A data point is a pair of input and output values, the total number $N$ of data points is the number of data points per system behaviour multiplied by the number of behaviours. %A data point is a pair of input and output values. 
The NN accuracy is defined by the {\em training} and {\em validation errors}, that are obtained from the loss function.   %$u$ corresponds to the control variable.

%% Nikos: @Thao, this is what i had written for the part.  


%
%\paragraph{Problem Formulation.} Given a nominal controller set and a plant, construct a sequence of neural nets $\neuralnet_i$,  training sets $\dataset_i$ and test sets $\testset_i$ such that, under some assumptions about the plant dynamics, eventually (for some $i$) when 


In what follows, we provide the main steps of our algorithm for designing a NN controller by iteratively constructing a sequence of neural nets $\neuralnet_i$, retraining sets $\dataset_i$ and test sets $\testset_i$ such that the final NN controller passes the specification test.
Furthermore, under some assumptions about the plant dynamics and robustness of nominal controllers, it is possible to guarantee that the algorithm always terminates with a correct NN controller. This algorithm relies on a coverage-based and counterexample based method for data generation that we will detail next. 

%\comment{Check how to nuance... We start with a nominal controller set $\controllerSet$ consisting only of a single controller $C_{\mathcal{S}}$ designed for the whole set $\mathcal{S}$ of control settings. During the design process, if this controller is not able to handle some control settings, a new nominal controller will be designed for these control settings and will be added to $\controllerSet$.}

\subsection{Coverage-Based Data Generation}\label{sec:covData}
%Note that in our case, the desired behaviours are produced by the nominal controllers. In order to create an initial NN controller, we sample a number of desired behaviours to have a good coverage of what the NN should learn. This will be discussed in more detail in Section~\ref{sec:covData}.

%{\color{red}REVIEW Another issue with the method is its practical application. The method requires the definition of an initial state, thus if training is done on a real system, this will be very cumbersome to do. Additionally, there are some scalability questions. While the paper is mentioning an application to a robotic arm (which itself is a bit misleading, since the robotic arm has only 2 states rendering it a simple pendulum), the system in question is still very small and it is unclear how the method scales with the size of the problem. => DONE}

In order to achieve a robust NN controller, we need to provide data representing diverse control settings that the NN should learn to cope with. Note that the set $\mathcal{S}$ of all possible control settings is generally infinite, we thus use a measure that quantifies how well a finite set of control settings covers the set $\mathcal{S}$. Considering the initial state $x_0$ as a constant signal having values in a given range, the set $\mathcal{S}$ can be treated as a continuous-time signal space. Let us now describe this measure, which is inspired by the notions of $\varepsilon$-entropy and  $\varepsilon$-capacity used to characterise the complexity of a function set~\cite{kolmogorov1959varepsilon}. We consider a continuous-time signal space $\sigspace$ where $\sigdom \subset \reals_+$ is the time domain of the signals in $\sigspace$. To capture the distance between two signals $u, w\in \sigspace$ we use the metric \begin{equation}\label{eq:distSig}
\distSig(u, w) = sup_{t \in \sigdom} |u(t)-w(t)|
\end{equation}
where $|\cdot|$ denotes the infinity norm.
Let $\sigset$ be a set of signals in $\sigspace$ %\is{very difficult to distinguish $\sigset$ and $\sigspace$}\td{I have changed the bold Sigma to bold Gamma.}  
that represents a class of signals of interest (such as reference signals, or expected temporal behaviours). 
\begin{itemize}
\item We call a signal set $\sigset_n$ an {\em $\varepsilon$-net} of $\sigset$ if for each element $r \in \sigset$, there exists $r'  \in \sigset_n$ such that $\distSig(r, r') \le \varepsilon$. 
\item A set $\sigset_s$ of signals in $\sigset$ is said {\em $\delta$-separated} if for all elements $r, r' \in \sigset_s$, $\distSig(r, r') >\delta$. 
\end{itemize}
%\myworries{Will it make more sense to use some other symbol like $\delta$ instead of $\varepsilon$ in the second item? Their values in general will be different, no? Thao: Indeed there is a link between the minimal eps-net and 2eps-separated set for some usual function classes. But we do not mention this so it makes sense to use different symbols. I changed it.}
Now for a given (possibly infinite) set $\sigset$ of signals in $\sigspace$, a finite $\varepsilon$-net of $\sigset$ and a $\delta$-separated subset of $\sigset$ can be combined to approximate the set $\sigset$. An  $\varepsilon$-net assures the ``coverage'' of the set $\sigset$, but by definition it may contain functions which are not in $\sigset$. A $\delta$-separated set is guaranteed to be a subset of $\sigset$ and the separation requirement aims at limiting the cardinality of the approximate sets, which will be used later in Section
~\ref{sec:cexDataGen} to select from a set of similar behaviours only a number of representative ones. 

%\is{Is it possible to add a picture here?}

In~\cite{kolmogorov1959varepsilon}, a method for constructing a minimal $\varepsilon$-net of a set of Lipschitz and smooth classes of functions is described. Here we are interested in the class of piece-wise constant signals which are suitable to represent reference signals in the control settings under consideration. We propose a simple grid-based method to construct $\varepsilon$-nets and sets satisfying some separation requirement. The set $\sigset$ of reference signals of our interest contains piece-wise constant signals with a fixed number of pieces $m$ of equal duration. For simplicity of explanation we assume that the signals are one dimensional and omit the set $X_0$ of initial conditions  (which can be considered, as mentioned earlier, as a constant signal). Let $[\underline{r}, \overline{r}]$ be the range of the reference signal. We use a grid $\mathcal{G}$ to partition the box $B_r = [\underline{r}, \overline{r}]^{m}$ into a set $G$ of rectangular cells with equal side length $2\varepsilon$ (assuming for simplicity that $(\overline{r} - \underline{r})/(2\varepsilon)$ is integral). Each point $p$ in this box $B_r$ corresponds to a signal in $\sigset$ defined as:  $r(t) = p_i$ for $t \in [t_i, t_{i} + \sigdom/m)$ with $i=0, 1, \ldots, (m-1)$ and $t_0=0$. In other words, the signal takes the $i^{th}$ coordinate of $p$ during the $i^{th}$ time interval. We denote by $\beta$ this mapping from a point $p \in B_r$ to $r \in \sigset$, and $\beta
^{-1}$ the mapping in the opposite direction. 
\begin{proposition}
Let $P$ be the set of center points of all the cells in $G$. The signal set $\sigset_n = \{ \beta(p) ~|~ p \in P \}$ is an $\varepsilon$-net of $\sigset$.
\end{proposition}
It is easy to see that any signal $u$ in $\sigset$ corresponds to a point $p_u$ in $B_r$. Let $p_w$ be the center point of the grid cell that contains $p_u$. Thus, $p_u$ is at distance (defined by the infinity norm) less than $\varepsilon$ to $p_w$, which $p_w$ in turn corresponds to a signal in $\sigset_n$. It indeed can be proved that $\sigset_n$ is a $\varepsilon$-net with minimal cardinality and also a $2\varepsilon$-separated set with maximal cardinality (this cardinality determines the $\varepsilon$-entropy and $2\varepsilon$-capacity of $\sigset$~\cite{kolmogorov1959varepsilon}). The data generation can be done using such an $\varepsilon$-net to guarantee a coverage of level at least $\varepsilon$. However, as we shall see later, to find counterexamples, the falsification process uses optimization algorithms which can explore many control settings within a grid cell. To have a coverage measure that better reflects the portion of the tested control settings, we use a finer grid $\mathcal{G}_c$ and take the ratio between the number of cells visited by both the sampling and falsification procedures and the total number of cells in this grid $\mathcal{G}_c$.   



%We use a measure called cell occupancy based on the ratio between the number $\occupiedcellcount$ of cells occupied by points and the total number $\numpartition$ of cells. Then, the cell occupancy measure is given as $\displaystyle{ \frac{\log \occupiedcellcount}{\log \numpartition}}$. Logarithm functions are used because the total number of cells could be very large as compared to the number of occupied cells. A major advantage of the cell-occupancy measure is that it is easy to compute; however, it is clear that when the cell size is large this measure does not reflect levels of uniformity or equi-distributivity, as provided by the Kolmogorov-Smirnov statistic~\cite{NFM19}. %The logarithms provide two key features for the cell occupancy measure: (1) they maintain the monotonicity of the measure, and (2) they result in reasonable measure values even for cases where the dimension $\cpdim$ is  large. 

% \subsection{NN Controller Validation and Counterexample Guided Neural Net Retraining}
\subsection{Counterexample Guided Retraining}
\label{sec:cexDataGen}
%\is{We can write counterexample instead of counterexample.}

Formal verification of the closed-loop system is generally difficult, as discussed in the introduction, since the composition of the neural net and the plant results in hybrid dynamics either with a large number of discrete modes caused by non-smooth activation functions or with stiff nonlinear continuous dynamics in high dimensions. Instead we try to quickly detect if the NN controller violates the expected closed-loop specification $\phi$, using a falsification method to check $( \neuralnet || \plant) \models \phi$. An outline of the methodology is shown in Figure~\ref{fig:methodology}.

A {\em counterexample} (\emph{cex} for short) is a behaviour that does not satisfy the specification. Behaviors that do satisfy  the specification are called {\em examples}. If no counterexample is found, we report the coverage of the set of explored control settings (see Section~\ref{sec:covData}). Otherwise, let $\counterexSet$ be the set of counterexamples that are found.
For each counterexample $\counterex \in \counterexSet$, we extract training data as follows: We use the control setting $s$ of $\counterex$ to simulate the corresponding nominal trajectory $\traj_s$ of $(\controllerSet || \plant)$, which represents a desired behaviour from which we extract the data $\data_{\traj_s}$ as in~\eqref{eq:dataextraction}.
%\myworries{[Adapting this paragraph based on the experimental result on the switched controller]....   If the corresponding nominal trajectory $\traj^{\controllerSet}_s \not \models \phi$, design a nominal controller $C_{\neigh(s)}$ for a neighbourhood $S = \neigh(s)$ of $s$, refine/subdivide the control setting set $\mathcal{S}$ accordingly, and then update the nominal local controller set $\controllerSet$ with this new (local) nominal controller $C_{\neigh(s)}$. Simulate again the corresponding nominal trajectory $\traj^{\controllerSet}_s$ of the closed loop with the updated controller set. Note that now $\traj^{\controllerSet}_s \models \phi$.} 
Besides the data from the counterexamples, we can add the data from a number of new examples ($E$) which are sampled or explored during the falsification process. With the new data set $\dataset$, we retrain the neural net $\neuralnet$.
To check whether the newly trained NN controller is satisfactory, we consider two types of checks: {\em matching quality} and {\em generalisation quality}. Concerning {\em matching quality}, we check if the neural net $\neuralnet$ has learnt well from the training data, meaning that for the control settings in the data set $\dataset$ that is used to train it, the closed loop $(\neuralnet || \plant)$ satisfies $\phi$. Concerning {\em generalisation quality},we check if $\neuralnet$ can generalise well, meaning that for the control settings not in the data set $\dataset$, the closed loop $(\neuralnet || \plant)$ still satisfies $\phi$.

%\ab{@GF do you maybe want to use figure 1 here? Feel free to suggest changes to the figure.}
%\gf{Yes, perfect!}
\begin{figure*}[t]
    \centering
    \includegraphics[scale=0.9]{figures/work-flow.eps}
    \caption{\small Counterexample Guided Neural Network Controller Retraining Methodology}
    \label{fig:methodology}
\end{figure*}

One iteration of the loop of retraining the NN controller is shown in Algorithm~\ref{algo:dataextraction}. Indeed, during the validation process, examples, that are trajectories satisfying the property, are generated and can be integrated in the data set for the next training. Let $\neuralnet_i$ be the neural network at the $i^{th}$ iteration.  

\begin{algorithm}[t]
\SetAlgoLined
\KwResult{Retrain from $\neuralnet_{i}$ to obtain $\neuralnet_{i+1}$}
\begin{algorithmic}
\STATE $\counterexSet_m \gets Test(\neuralnet_i || \plant, \dataset_{i}, \; \phi)$   
\texttt{/* matching test  */}\\
\STATE $\langle \counterexSet_g, E\rangle \gets Test(\neuralnet_i|| \plant, \; \overline{\dataset}_i, \; \phi)$ \texttt{/* generalisation test, $\overline{\dataset}_i$ is the complement of $\dataset_i$ */}~\\
%\STATE $\counterexSet_g  \gets Test(\neuralnet_i|| \plant, \; \phi)$ \texttt{/* generalisation test via falsification}~\\
\STATE $\counterexSet \gets \counterexSet_m \cup \counterexSet_g$ 
\texttt{/* collecting all the counterexamples */} ~\\
\STATE $\dataset_{i}^S\gets Process_{cex}(\counterexSet)$
\texttt{/* processing counterexample via clustering */} ~\\
%%% OLD with examples
%\STATE $\dataset_{i}^S\gets Select_{cex}(\counterexSet) \cup Select_{ex}(\exampleSet)$ 
%\texttt{/* counterexample selection and example processing */} ~\\
\STATE $\dataset_{i}^E\gets Process_{ex}(E)$
\texttt{/* processing examples */} ~\\
\STATE $\dataset_{i+1} \gets  \dataset_{i} \cup \dataset_{i}^S \cup \dataset_{i}^E$
\texttt{/* update the data set */}~\\
%\STATE $\dataset_{i+1} \gets  \dataset_{i} \cup Select_{cex}(\counterexSet) \cup Select_{ex}(\exampleSet)$ 
%\texttt{/* update the data set */}~\\
%\is{Should we not show the clustering step in the algorithm?}
\STATE $\neuralnet_{i+1} \gets Training(\neuralnet_{i},\dataset_{i+1})$ 
\texttt{/* retraining with the updated data set */}\\
\end{algorithmic}
\caption{Neural Net Retraining using Falsification}
\label{algo:dataextraction}
\end{algorithm}


% \begin{algorithm}[t]
% \SetAlgoLined
% \KwResult{Retrain from $\neuralnet_{i}$ to obtain $\neuralnet_{i+1}$}
% \begin{algorithmic}
% \STATE $\counterexSet_m \gets Test(\neuralnet_i || \plant, \dataset_{i}, \; \phi)$   
% \texttt{/* matching test  */}\\
% % \STATE $\counterexSet_g \cup \exampleSet \gets Test(\neuralnet_i|| \plant, \; \overline{\dataset}_i, \; \phi)$ \texttt{/* generalisation test, $\overline{\dataset}_i$ is the complement of $\dataset_i$ */}~\\
% \STATE $\counterexSet_g  \gets Test(\neuralnet_i|| \plant, \; \phi)$ \texttt{/* generalisation test via falsification}~\\
% \STATE $\counterexSet \gets \counterexSet_m \cup \counterexSet_g$ 
% \texttt{/* collecting all the counterexamples */} ~\\
% \STATE $\dataset_{i}^S\gets Select_{cex}(\counterexSet)$
% \texttt{/* counterexample processing via clustering */} ~\\
% %%% OLD with examples
% %\STATE $\dataset_{i}^S\gets Select_{cex}(\counterexSet) \cup Select_{ex}(\exampleSet)$ 
% %\texttt{/* counterexample selection and example processing */} ~\\
% \STATE $\dataset_{i+1} \gets  \dataset_{i} \cup \dataset_{i}^S$
% \texttt{/* update the data set */}~\\
% %\STATE $\dataset_{i+1} \gets  \dataset_{i} \cup Select_{cex}(\counterexSet) \cup Select_{ex}(\exampleSet)$ 
% %\texttt{/* update the data set */}~\\
% %\is{Should we not show the clustering step in the algorithm?}
% \STATE $\neuralnet_{i+1} \gets Training(\neuralnet_{i},\dataset_{i+1})$ 
% \texttt{/* retraining with the updated data set */}\\
% \end{algorithmic}
% \caption{Neural Net Retraining using Falsification}
% \label{algo:dataextraction}
% \end{algorithm}

The first test is a matching quality test on the control settings in the data set $\dataset_{i}$ used for training $\neuralnet_i$. This check can generate a set $\counterexSet_m$ of {\em matching counterexamples}. 
The second check concerns generalisation quality, which can be defined as the ability of a trained NN to deal with situations which were not seen during training. Note that a trained NN may not generalise well because it is subject to over-fitting (that is, it essentially memorizes the training data, and indeed performs with high accuracy on the seen data but poorly on unseen data). To test the generalisation ability of a NN controller, in the $(i+1)^{th}$ iteration, we generate a set of control settings which are not in $\dataset_i$ (denoted by $\overline{\dataset}_i$) and test the current NN controller under these settings. 
To implement this generalization test procedure, we use a falsifier (e.g., Breach~\cite{breach}) where we restrict the set of explored control settings to $\overline{\dataset}_i$.
This test generates a set $\counterexSet_g$ of {\em generalisation counterexamples} and a set $E$ of examples (satisfying trajectories). 
% The procedure $Select_{cex}(\counterexSet)$ extracts data from the sets of counterexamples to  fulfil the objective of \emph{exploitation} (keeping similar counterexamples for counterexample elimination) and diversification. 
%%ORIGINAL
%This test generates a set $\exampleSet$ of examples (that is satisfying trajectories) and a set $\counterexSet_g$ of {\em generalisation counterexamples}. 
The procedures $Process_{cex}(\counterexSet)$ and $Process_{ex}(E)$ extract data from the sets of counterexamples and examples so as to fulfil two objectives: exploitation (keeping similar counterexamples for counterexample elimination) and diversification (keeping diverse examples for generalisation enhancement). 
 To this end, we propose a behaviour clustering technique.  This technique is based on a measure of distance between control settings: given two control settings $s=(x_0,r
(\cdot))$ and $s'= (x'_0,r'
(\cdot), \dis(\cdot))$, $\csdist(s, s') = | (x_0, \beta^{-1}(r)) -  (x'_0, \beta^{-1}(r))| $. 
We use silhouette analysis to estimate first an optimal number of clusters which is then used to cluster the behaviours via the k-means algorithm. Then, to form a new data set, we select a subset of behaviours in each cluster, using two criteria: (1) the selected behaviours are separated by a given amount $\delta$ (for diversification purposes), (2) the robustness values of the selected behaviours are among $K_{\rho}$ worst values (for exploitation purposes).  

 \begin{proposition}\label{prop:trajError}
Let $\neuralnet$ be a neural net trained using the data set $\dataset$.  Let $\dataset'= \dataset \cup \data_{\traj_s}$ where $\data_{\traj_s}$ be data corresponding to a new desired closed-loop behaviour $\traj_s$ under a control setting $s$. Let $\neuralnet'$ be the new net trained using  $\dataset'$ and $\traj'_s$ be the behaviour of $(\neuralnet' || \plant)$ under the control setting $s$. If the training error of $\neuralnet'$ is bounded by $\epsilon$, then there exists bounded $\eta$ depending on $\epsilon$ such that  $\distSig(\traj_s, \traj'_s)  \le \eta$ where the distance metric $\distSig$ is defined in \eqref{eq:distSig}.
\end{proposition}  
The proof of the proposition relies on the Lipschitz continuity of the plant dynamics and can be found in Appendix.




%\cite{TR-VerimagKanpur2020}.
The above proposition shows that if we can train the neural net with arbitrary accuracy, then for a given control setting we can train the neural net to make the system follow a desired closed-loop behaviour as closely as we want. In other words, it is possible to eliminate a counterexample corresponding to a control setting $s$, we can choose for the same control setting a desired behaviour which is sufficiently robust. Training the neural net with the data from this desired behaviour allows eliminating the counterexample in question.


==> iccps2023_version/cex_guided_algo.tex <==
\section{Closed-Loop Specification Guided Approach for NN Controller Learning}

%\is{This section is too long. Perhaps we could split it into two sections: Problem (Section 3.1 and 3.2) and Algorithm (Section 3.3, 3.4, 3.5).}22
%Broad outline of the algorithm
%Stress on the face that we use STL to check correctness
%Stress on the use of closed-loop analysis
%Abstract away details of tools used (Breach)

\subsection{Problem Setting}
We consider a continuous-time plant $\Pi$ with state $x \in \reals^n$ that is controlled by an input signal $u$, observed through an output signal $y$, and disturbed by an external signal $\dis$ with dynamics
\begin{eqnarray}
\dot{x}(t)  &=&  f(x(t), u(t), \dis(t)), \label{eq:1}\\
y(t) & = & \zeta(x(t))\nonumber.
\end{eqnarray}
%\is{For the MPC model, we need to introduce disturbance in this equation.}
%\nk{d}
%where $u$ is the control input and $y$ is the plant output. 
The control input $u$ is computed by 
a \emph{nominal} discrete-time controller $\mathcal{C}$ with state $z \in \reals^{n_z}$ %\ih{what is $n_z$ here? Do we need to define it?}
\begin{eqnarray}\label{eq:controller}
z_{k+1} &= & f_c(z_k, y_k, r_k), \\
u_k &= & \upsilon(z_k, y_k,r_k)
\end{eqnarray}
where $r_k$ and $y_k$ are discrete-time signals resulting from sampling the reference $r(\cdot)$ and the output $y(\cdot)$ with a constant time step $\timestep$, that is $\forall k = 0, 1, 2, \ldots, r_k = u(k\timestep), y_k = y(k\timestep)$. The continuous-time control $u(\cdot)$ is a piece-wise constant function defined as $\forall t \in [k\timestep, (k+1)\timestep)~ u(t) = u_k$ with $k = 0, 1, \ldots$. Starting from an initial state $x(0)=x_0 \in X_0$, the behaviour of the system is a vector of functions $\traj=(r(\cdot), x(\cdot), u(\cdot), y(\cdot), \dis(\cdot))$ that satisfies the system equations. We use the usual Lipschitz assumptions about the function $f$ so as to guarantee the existence and uniqueness of the solution. We introduce the notion of ``control setting'' to refer to a pair $s= (x_0, r(\cdot),\dis(\cdot))$ where $x_0$ is the initial state of the plant, $r(\cdot)$ is the reference signal, and $\dis(\cdot)$ is the disturbance signal. Let $\mathcal{S}$ denote the set of all possible control settings. Under each control setting $s$, the controller (represented by the function $f_c$) generates a behaviour, and for convenience we denote it by $\traj_s$. %For example, $x_0=(p(0), v(0))$ where $p(0)$ and $v(0)$ are the initial position and speed of a robot; $(p, v)$ may be only partial state of the plant. \myworries{examples of reference signals}
 
% We assume that we have a method of designing a nominal controller $C$ for the plant in some set $S$ of control settings, that is, for every $s=(x_0, r(\cdot)) \in S$ this controller can make the output $y$ of the plant, starting at the initial condition $x_0$ under the reference input signal $r(\cdot)$), track the reference $r$ while satisfying a property $\phi$ (specified by a temporal logic for example). The property $\phi$ can be, for example, reaching a goal point while satisfying some transient response specifications. As we shall see, the validity of this control design assumption will also be checked during our design process. 

Our goal is to generate a NN feedback controller so that the closed-loop system satisfies some desired properties, where the learning guidance is provided using positive examples, that is good behaviours. This learning-based approach is of particular interest when good behaviours cannot be generated by a single control law but only by combining different control laws. Indeed, when the plant is nonlinear, it is hard to find one controller of a fixed structure (such as PID, MPC) that performs well for all control settings, and it is 
time-consuming to fine-tune the parameters to adapt to new scenarios. Here we can see the interest of using NN controllers as a means of combining controllers. Indeed, by exploiting the approximation power of NN, they can be trained to achieve the qualities that are difficult to achieve jointly using conventional control methods. 

%\subsection{Nominal Controllers}
%We assume that we are given a nominal controller $C$ that can produce a desired closed-loop behaviour (satisfying the control specification) for every control setting $s=(x_0, r(\cdot)) \in S$. 
%In the remainder of the paper, let $C$ denote a nominal controller designed for every control setting $s=(x_0, r(\cdot)) \in S$. 
In the learning context, a nominal controller plays the role of a teacher that generates a desired closed-loop behaviour for a given control setting which the NN should learn. To do so, the nominal controller makes use of a collection of conventional controllers, each of which is responsible for a subset of control settings or satisfies a subset of desired control properties. In this paper we focus only on the problem of how to iteratively train NN using examples (good behaviours) and counterexamples (bad behaviours). A method for generating good behaviours combining different properties from a collection of controllers is illustrated via an example described in Sect.\;\ref{sec:experiment}.

\subsection{Control Specifications}
Our control objective is to make the output $y$ of the plant, starting at an initial condition $x_0 \in X_0$, track the reference $r$ while satisfying a property $\phi$ specified using STL. Before recalling STL, we remark that our framework deals with finite-time traces which cannot be used to prove liveness and stability properties. However, practical stability, such as convergence to a region (for example a neighbourhood of the origin) during a given time interval~\cite{Lasalle61}, has been intensively studied in theory and proven useful in practice. Furthermore, combining with invariant computation, finite-time traces can be used to falsify liveness properties (such as by showing the system will get trapped in some set after some finite time~\cite{Navarro-LopezC16}). STL and temporal logics in general have been used by the control community to specify various control performance properties~\cite{AMT20_2018}. Some examples of typical control specifications expressed in STL can be found in Sect.\;\ref{sec:experiment}.

\input{stl.tex} 

%{\color{red} REVIEW => DONE
%- When a continuous control is implemented via sampled systems in safety critical applications, they use adaptive sampling frequencies where the schedule of sampling is certified to not miss critical events. There appears to be a fundamental flaw here in realizing that when designing safe systems with formal specifications, these differences in continuous-time and discrete-time applications matter significantly. 
%- There is a conflation of terminology leading to some overstatement of the value of temporal properties in this paper. Temporal logic properties considered in the paper are limited to have fixed windows. This eliminates much of the strength of temporal logic in stating properties such as liveness and eventual convergence or orbit (cycle) behavior. In fact, simple trace distance metrics would be able to model this kind of STL properties (and be in fact more expressive - something akin to robustness metric of STL). This restricted form of STL properties is not sufficient to express specifications of stability, convergence and the other interesting properties useful in control systems. Discrete-time nature of these properties can have some applications but these restrictions should be mentioned earlier to make the contribution of this paper more clear. The use of really small time bounds in the experiment section further makes the reviewer less convinced that the presented technique can handle useful practical properties.}

%{\color{red}REVIEW: However, no empirical evidence is provided to support this claim, and the theoretical argument seems to rest on the assumption that the NN can be trained to arbitrary accuracy.It is unclear if this claim can hold with the given method, since in the various data collection steps ultimately the trajectory to be imitated is being generated by the nominal controller. Furthermore, the nominal controller is assumed to satisfy all the STL properties proposed in Section 4. Thus a-priori we would assume that the NN controller would not outperform the nominal controller.


%Additionally, a key issue of the method is not addressed: Is the retrained and robustified NN controller better than the nominal controller? Especially, if the predefined properties are restrictive, there are a lot of counter examples and the behavior of the NN controller converges to the behavior of the nominal controller. As seen in the numerical example, the NN controller is unable to outperform the simple PID controller, which raises the question: ”What is the motivation to use the new approach over a simple, cheap, and easy-to-tune PID controller? One possible motivation is mentioned in the introduction, namely to merge multiple controllers - which work in some parts of the state space - into one controller. However, this point is never picked up again in the remainder of the paper.

%What is the value of learning DNN controller from a nominal controller? Why can't such a translation, if needed, be accomplished more efficiently through rewrite based compilation (incrementally replace expressions with DNN equivalents)? => DONE


%"produce NN controllers that are able to combine the qualities of a set of nominal controllers such that no single controller can guarantee" - This claim is not justified by any theorem in the paper. Even an intuitive argument would have been useful. => DONE

%- One major assumption is that training a DNN controller is useful when one already has a nominal controller. And even if this change in representation is useful, why not directly compile the controller into DNN using rewrite rules rather than train using examples. => DONE}

%It is of interest to combine a number of nominal controllers, each controller $C_S$ is designed for a set $S \subseteq \mathcal{S}$ of control settings such that the union of all such sets $S$ covers the set $\mathcal{S}$ of all possible control settings. The set of all such controllers is called {\em nominal controller set} $\controllerSet = \{ C_S ~|~ S \subseteq \mathcal{S} ~\land~ \mathcal{S} \subseteq \bigcup S \}$. \myworries{adapt the speech if the switching controller example can be handled}


%The validity of this control design assumption will also be checked during our design process.

\subsection{Neural Net Structure and Training} Intuitively, the NN controller is trained based on the desired closed-loop behaviours we want it to learn. Let $\traj = (r(\cdot), x(\cdot), u(\cdot), y(\cdot), \dis(\cdot))$ be a desired closed-loop behaviour, from which we extract the data of the form \begin{equation}\label{eq:dataextraction}
\data_{\traj} = \bigl\{ (r_k, y_k, u_k, \dis_k) \bigm| k < K \bigr\}
\end{equation}
where $r_k$, $y_k$, $u_k$, and $d_k$ are respectively the reference value, output value and control value at time $t_k$; $K$ is the discrete time horizon (that is, the number of sampled time points). When many desired behaviours are considered, the data set $\dataset$ is the union of all $\data_{\traj}$. We generate a neural net $\neuralnet$ to match the data set $\dataset$. The structure of the NN should capture the input-output relationship of the controller in \eqref{eq:controller}. We add past values to represent the memory needed to compute the output at each discrete step. The input of the neural net is
$(r_k, r_{k-1},\ldots, r_{k-n_r}, \overline{y}_k, \overline{y}_{k-1}, \ldots, \overline{y}_{k-n_y}, \overline{u}_{k-1}, \ldots, \overline{u}_{k-n_u})$ where $n_r$,$n_y$, $n_u$ represent the number of previous values (memory) of $r_k$, $y_k$, $u_k$ respectively that are needed for training, and the output is $\overline{u}_k$.  To train the NN, we use a loss function defined via the Mean Square Error (MSE): ${\frac{1}{N}\sum_{k=1}^N (u_k-\overline{u}_k)^2}$, where $u$ is the output of the nominal controller and $\overline{u}$ is the output of the NN. A data point is a pair of input and output values, the total number $N$ of data points is the number of data points per system behaviour multiplied by the number of behaviours. %A data point is a pair of input and output values. 
The NN accuracy is defined by the {\em training} and {\em validation errors}, that are obtained from the loss function.   %$u$ corresponds to the control variable.

%% Nikos: @Thao, this is what i had written for the part.  


%
%\paragraph{Problem Formulation.} Given a nominal controller set and a plant, construct a sequence of neural nets $\neuralnet_i$,  training sets $\dataset_i$ and test sets $\testset_i$ such that, under some assumptions about the plant dynamics, eventually (for some $i$) when 


In the following, we give the main steps of our algorithm for designing a NN controller by iteratively constructing a sequence of neural nets $\neuralnet_i$, retraining sets $\dataset_i$ and test sets $\testset_i$ such that the final NN controller passes the specification test.
Furthermore, under some assumptions about the plant dynamics and robustness of nominal controllers, it is possible to guarantee that the algorithm always terminates with a correct NN controller. This algorithm relies on a coverage-based and counterexample based method for data generation that we will detail in the following. 

%\comment{Check how to nuance... We start with a nominal controller set $\controllerSet$ consisting only of a single controller $C_{\mathcal{S}}$ designed for the whole set $\mathcal{S}$ of control settings. During the design process, if this controller is not able to handle some control settings, a new nominal controller will be designed for these control settings and will be added to $\controllerSet$.}

\subsection{Coverage-Based Data Generation}\label{sec:covData}
%Note that in our case, the desired behaviours are produced by the nominal controllers. In order to create an initial NN controller, we sample a number of desired behaviours to have a good coverage of what the NN should learn. This will be discussed in more detail in Section~\ref{sec:covData}.

%{\color{red}REVIEW Another issue with the method is its practical application. The method requires the definition of an initial state, thus if training is done on a real system, this will be very cumbersome to do. Additionally, there are some scalability questions. While the paper is mentioning an application to a robotic arm (which itself is a bit misleading, since the robotic arm has only 2 states rendering it a simple pendulum), the system in question is still very small and it is unclear how the method scales with the size of the problem. => DONE}

In order to achieve a robust NN controller, we need to provide data representing diverse control settings that the NN should learn to cope with. Note that the set $\mathcal{S}$ of all possible control settings is generally infinite, we thus use a measure that quantifies how well a finite set of control settings covers the set $\mathcal{S}$. Considering the initial state $x_0$ as a constant signal having values in a given range, the set $\mathcal{S}$ can be treated as a continuous-time signal space. Let us now describe this measure, which is inspired by the notions of $\varepsilon$-entropy and  $\varepsilon$-capacity used to characterise the complexity of a function set~\cite{kolmogorov1959varepsilon}. We consider a continuous-time signal space $\sigspace$ where $\sigdom \subset \reals_+$ is the time domain of the signals in $\sigspace$. To capture the distance between two signals $u, w\in \sigspace$ we use the metric \begin{equation}\label{eq:distSig}
\distSig(u, w) = sup_{t \in \sigdom} |u(t)-w(t)|
\end{equation}
where $|\cdot|$ denotes the infinity norm.
Let $\sigset$ be a set of signals in $\sigspace$ %\is{very difficult to distinguish $\sigset$ and $\sigspace$}\td{I have changed the bold Sigma to bold Gamma.}  
that represents a class of signals of interest (such as reference signals, or expected temporal behaviours). 
\begin{itemize}
\item We call a signal set $\sigset_n$ an {\em $\varepsilon$-net} of $\sigset$ if for each element $r \in \sigset$, there exists $r'  \in \sigset_n$ such that $\distSig(r, r') \le \varepsilon$. 
\item A set $\sigset_s$ of signals in $\sigset$ is said {\em $\delta$-separated} if for all elements $r, r' \in \sigset_s$, $\distSig(r, r') >\delta$. 
\end{itemize}
%\myworries{Will it make more sense to use some other symbol like $\delta$ instead of $\varepsilon$ in the second item? Their values in general will be different, no? Thao: Indeed there is a link between the minimal eps-net and 2eps-separated set for some usual function classes. But we do not mention this so it makes sense to use different symbols. I changed it.}
Now for a given (possibly infinite) set $\sigset$ of signals in $\sigspace$, a finite $\varepsilon$-net of $\sigset$ and a $\delta$-separated subset of $\sigset$ can be combined to approximate the set $\sigset$. An  $\varepsilon$-net assures the ``coverage'' of the set $\sigset$, but by definition it may contain functions which are not in $\sigset$. A $\delta$-separated set is guaranteed to be a subset of $\sigset$ and the separation requirement aims at limiting the cardinality of the approximate sets, which will be used later in Section
~\ref{sec:cexDataGen} to select from a set of similar behaviours only a number of representative ones. 

%\is{Is it possible to add a picture here?}

In~\cite{kolmogorov1959varepsilon}, a method for constructing a minimal $\varepsilon$-net of a set of Lipschitz and smooth classes of functions is described. Here we are interested in the class of piece-wise constant signals which are suitable to represent reference signals in the control settings under consideration. We propose a simple grid-based method to construct $\varepsilon$-nets and sets satisfying some separation requirement. The set $\sigset$ of reference signals of our interest contains piece-wise constant signals with a fixed number of pieces $m$ of equal duration. For simplicity of explanation we assume that the signals are one dimensional and omit the set $X_0$ of initial conditions  (which can be considered, as mentioned earlier, as a constant signal). Let $[\underline{r}, \overline{r}]$ be the range of the reference signal. We use a grid $\mathcal{G}$ to partition the box $B_r = [\underline{r}, \overline{r}]^{m}$ into a set $G$ of rectangular cells with equal side length $2\varepsilon$ (assuming for simplicity that $(\overline{r} - \underline{r})/(2\varepsilon)$ is integral). Each point $p$ in this box $B_r$ corresponds to a signal in $\sigset$ defined as:  $r(t) = p_i$ for $t \in [t_i, t_{i} + \sigdom/m)$ with $i=0, 1, \ldots, (m-1)$ and $t_0=0$. In other words, the signal takes the $i^{th}$ coordinate of $p$ during the $i^{th}$ time interval. We denote by $\beta$ this mapping from a point $p \in B_r$ to $r \in \sigset$, and $\beta
^{-1}$ the mapping in the opposite direction. 
\begin{proposition}
Let $P$ be the set of center points of all the cells in $G$. The signal set $\sigset_n = \{ \beta(p) ~|~ p \in P \}$ is an $\varepsilon$-net of $\sigset$.
\end{proposition}
It is easy to see that any signal $u$ in $\sigset$ corresponds to a point $p_u$ in $B_r$. Let $p_w$ be the center point of the grid cell that contains $p_u$. Thus, $p_u$ is at distance (defined by the infinity norm) less than $\varepsilon$ to $p_w$, which $p_w$ in turn corresponds to a signal in $\sigset_n$. It indeed can be proved that $\sigset_n$ is a $\varepsilon$-net with minimal cardinality and also a $2\varepsilon$-separated set with maximal cardinality (this cardinality determines the $\varepsilon$-entropy and $2\varepsilon$-capacity of $\sigset$~\cite{kolmogorov1959varepsilon}). The data generation can be done using such an $\varepsilon$-net to guarantee a coverage of level at least $\varepsilon$. However, as we shall see later, to find counterexamples, the falsification process uses optimization algorithms which can explore many control settings within a grid cell. To have a coverage measure that better reflects the portion of the tested control settings, we use a finer grid $\mathcal{G}_c$ and take the ratio between the number of cells visited by both the sampling and falsification procedures and the total number of cells in this grid $\mathcal{G}_c$.   



%We use a measure called cell occupancy based on the ratio between the number $\occupiedcellcount$ of cells occupied by points and the total number $\numpartition$ of cells. Then, the cell occupancy measure is given as $\displaystyle{ \frac{\log \occupiedcellcount}{\log \numpartition}}$. Logarithm functions are used because the total number of cells could be very large as compared to the number of occupied cells. A major advantage of the cell-occupancy measure is that it is easy to compute; however, it is clear that when the cell size is large this measure does not reflect levels of uniformity or equi-distributivity, as provided by the Kolmogorov-Smirnov statistic~\cite{NFM19}. %The logarithms provide two key features for the cell occupancy measure: (1) they maintain the monotonicity of the measure, and (2) they result in reasonable measure values even for cases where the dimension $\cpdim$ is  large. 

\subsection{NN Controller Validation and Counterexample Guided Neural Net Retraining}\label{sec:cexDataGen}
%\is{We can write counterexample instead of counterexample.}

Formal verification of the closed-loop system is generally difficult, as discussed in the introduction, since the composition of the neural net and the plant results in hybrid dynamics either with a large number of discrete modes caused by non-smooth activation functions or with stiff nonlinear continuous dynamics in high dimensions. Instead we try to quickly detect if the NN controller violates the expected closed-loop specification $\phi$, using a falsification method to check $( \neuralnet || \plant) \models \phi$. An outline of the methodology is shown in Figure~\ref{fig:methodology}.

A {\em counterexample} (\emph{cex} for short) is a behaviour that does not satisfy the specification. Behaviors that do satisfy  the specification are called {\em examples}. If no counterexample is found, we report the coverage of the set of explored control settings (see Section~\ref{sec:covData}). Otherwise, let $\counterexSet$ be the set of counterexamples that are found.
For each counterexample $\counterex \in \counterexSet$, we extract training data as follows: We use the control setting $s$ of $\counterex$ to simulate the corresponding nominal trajectory $\traj_s$ of $(\controllerSet || \plant)$, which represents a desired behaviour from which we extract the data $\data_{\traj_s}$ as in~\eqref{eq:dataextraction}.
%\myworries{[Adapting this paragraph based on the experimental result on the switched controller]....   If the corresponding nominal trajectory $\traj^{\controllerSet}_s \not \models \phi$, design a nominal controller $C_{\neigh(s)}$ for a neighbourhood $S = \neigh(s)$ of $s$, refine/subdivide the control setting set $\mathcal{S}$ accordingly, and then update the nominal local controller set $\controllerSet$ with this new (local) nominal controller $C_{\neigh(s)}$. Simulate again the corresponding nominal trajectory $\traj^{\controllerSet}_s$ of the closed loop with the updated controller set. Note that now $\traj^{\controllerSet}_s \models \phi$.} 
Besides the data from the counterexamples, we can add the data from a number of new examples which are sampled or explored during the falsification process. With the new data set $\dataset$, we retrain the neural net $\neuralnet$.
To check whether the newly trained NN controller is satisfactory, we consider two types of checks: {\em matching quality} and {\em generalisation quality}. Concerning {\em matching quality}, we check if the neural net $\neuralnet$ has learnt well from the training data, meaning that for the control settings in the data set $\dataset$ that is used to train it, the closed loop $(\neuralnet || \plant)$ satisfies $\phi$. Concerning {\em generalisation quality},we check if $\neuralnet$ can generalise well, meaning that for the control settings not in the data set $\dataset$, the closed loop $(\neuralnet || \plant)$ still satisfies $\phi$.

%\ab{@GF do you maybe want to use figure 1 here? Feel free to suggest changes to the figure.}
%\gf{Yes, perfect!}
\begin{figure*}[t]
    \centering
    \includegraphics[scale=0.9]{figures/work-flow.eps}
    \caption{\small Counterexample Guided Neural Network Controller Retraining Methodology}
    \label{fig:methodology}
\end{figure*}

One iteration of the loop of retraining the NN controller is shown in Algorithm~\ref{algo:dataextraction}. Indeed, during the validation process, examples, that are trajectories satisfying the property, are generated and can be integrated in the data set for the next training. Let $\neuralnet_i$ be the neural network at the $i^{th}$ iteration.  
\begin{algorithm}[t]
\SetAlgoLined
\KwResult{Retrain from $\neuralnet_{i}$ to obtain $\neuralnet_{i+1}$}
\begin{algorithmic}
\STATE $\counterexSet_m \gets Test(\neuralnet_i || \plant, \dataset_{i}, \; \phi)$   
\texttt{/* matching test  */}\\
%\STATE $\counterexSet_g \cup \exampleSet \gets Test(\neuralnet_i|| \plant, \; \overline{\dataset}_i, \; \phi)$ \texttt{/* generalisation test, $\overline{\dataset}_i$ is the complement of $\dataset_i$ */}~\\
\STATE $\counterexSet_g  \gets Test(\neuralnet_i|| \plant, \; \phi)$ \texttt{/* generalisation test via falsification}~\\
\STATE $\counterexSet \gets \counterexSet_m \cup \counterexSet_g$ 
\texttt{/* collecting all the counterexamples */} ~\\
\STATE $\dataset_{i}^S\gets Select_{cex}(\counterexSet)$
\texttt{/* counterexample processing via clustering */} ~\\
%%% OLD with examples
%\STATE $\dataset_{i}^S\gets Select_{cex}(\counterexSet) \cup Select_{ex}(\exampleSet)$ 
%\texttt{/* counterexample selection and example processing */} ~\\
\STATE $\dataset_{i+1} \gets  \dataset_{i} \cup \dataset_{i}^S$
\texttt{/* update the data set */}~\\
%\STATE $\dataset_{i+1} \gets  \dataset_{i} \cup Select_{cex}(\counterexSet) \cup Select_{ex}(\exampleSet)$ 
%\texttt{/* update the data set */}~\\
%\is{Should we not show the clustering step in the algorithm?}
\STATE $\neuralnet_{i+1} \gets Training(\neuralnet_{i},\dataset_{i+1})$ 
\texttt{/* retraining with the updated data set */}\\
\end{algorithmic}
\caption{Neural Net Retraining using Falsification}
\label{algo:dataextraction}
\end{algorithm}
The first test is a matching quality test on the control settings in the data set $\dataset_{i}$ used for training $\neuralnet_i$. This check can generate a set $\counterexSet_m$ of {\em matching counterexamples}. The second check concerns generalisation quality, which can be defined as the ability of a trained NN to deal with situations which were not seen during training. Note that a trained NN may not generalise well because it is subject to over-fitting (that is, it essentially memorizes the training data, and indeed performs with high accuracy on the seen data but poorly on unseen data). To test the generalisation ability of a NN controller, in the $(i+1)^{th}$ iteration, we generate a set of control settings which are not in $\dataset_i$ and test the current NN controller under these settings. This test generates a set $\counterexSet_g$ of {\em generalisation counterexamples}. 
The procedure $Select_{cex}(\counterexSet)$ extracts data from the sets of counterexamples to  fulfil the objective of \emph{exploitation} (keeping similar counterexamples for counterexample elimination) and diversification. 
%%ORIGINAL
%This test generates a set $\exampleSet$ of examples (that is satisfying trajectories) and a set $\counterexSet_g$ of {\em generalisation counterexamples}. 
%The procedures $Select_{cex}(\counterexSet)$ and $Select_{ex}(\exampleSet)$ extract data from the sets of counterexamples and examples so as to fulfil two objectives: exploitation (keeping similar counterexamples for counterexample elimination) and diversification (keeping diverse examples for generalisation enhancement). 
 To this end, we propose a behaviour clustering technique.  This technique is based on a measure of distance between control settings: given two control settings $s=(x_0,r
(\cdot))$ and $s'= (x'_0,r'
(\cdot))$, $\csdist(s, s') = | (x_0, \beta^{-1}(r)) -  (x'_0, \beta^{-1}(r))| $. 
We use silhouette analysis to estimate first an optimal number of clusters which is then used to cluster the behaviours via the k-means algorithm. Then, to form a new data set, we select a subset of behaviours in each cluster, using two criteria: (1) the selected behaviours are separated by a given amount $\delta$ (for diversification purposes), (2) the robustness values of the selected behaviours are among $K_{\rho}$ worst values (for exploitation purposes).  

 \begin{proposition}\label{prop:trajError}
Let $\neuralnet$ be a neural net trained using the data set $\dataset$.  Let $\dataset'= \dataset \cup \data_{\traj_s}$ where $\data_{\traj_s}$ be data corresponding to a new desired closed-loop behaviour $\traj_s$ under a control setting $s$. Let $\neuralnet'$ be the new net trained using  $\dataset'$ and $\traj'_s$ be the behaviour of $(\neuralnet' || \plant)$ under the control setting $s$. If the training error of $\neuralnet'$ is bounded by $\epsilon$, then there exists bounded $\eta$ depending on $\epsilon$ such that  $\distSig(\traj_s, \traj'_s)  \le \eta$ where the distance metric $\distSig$ is defined in \eqref{eq:distSig}.
\end{proposition}  
The proof of the proposition relies on the Lipschitz continuity of the plant dynamics and can be found in Appendix.




%\cite{TR-VerimagKanpur2020}.
The above proposition shows that if we can train the neural net with arbitrary accuracy, then for a given control setting we can train the neural net to make the system follow a desired closed-loop behaviour as closely as we want. In other words, it is possible to eliminate a counterexample corresponding to a control setting $s$, we can choose for the same control setting a desired behaviour which is sufficiently robust. Training the neural net with the data from this desired behaviour allows eliminating the counterexample in question.


%\subsection{Running Example: --}\label{sec:runningExample}\myworries{todo}
% 3 part figure -
% A) Coverage for Initial Data Generation (example of a grid)
% B) Counterexamples from Breach - one plot of nominal behaviour
% C) Final Training Information (Initial PID, Initial NN, NN with no counterexamples, NN with random example based training) - Has to be on the same input reference


==> iccps2023_version/cex_selection_algo.tex <==
\begin{algorithm}[H]
\SetAlgoLined
\SetKwInOut{Input}{Input}
\Input{Counterexamples (traces) $\counterexSet$, Counterexamples robustness (scalar) $\rho_{cex}$, tolerance $e_{cex}$, cluster range $c_{range}$ \texttt{/* normally, $|max(c_{range})|=10$  \myworries{maximal nb of clusters} */}}
\KwResult{Obtain $\hat{\counterexSet}=Select_{cex}(\counterexSet)$ }
\begin{algorithmic}
\STATE $\counterexSet_{vec}=\{\counterexSet\downarrow \beta\}$ 
\texttt{/* Get vector of reference set-points from traces  */}\\
\STATE $n_{cluster}=Silhouette(\counterexSet_{vec}, c_{range})$ \texttt{/* optimal \#clusters via silhouette analysis  */}~\\
\STATE $Clusters_{1,\ldots,n_{cluster}}=Kmeans(\counterexSet_{vec},n_{cluster},'replicates',8,'Euclidean Distance')$ \texttt{perform k-means clustering with replicates}
\STATE \For{$i$=1 to $|\counterexSet_{vec}|$} {
$\counterexSet_{vec}^i\leftarrow assign(\counterexSet_{vec},Clusters,Centroids)$
\texttt{/* assign counterexamples to clusters with the minimum square error from the cluster centroid  */} ~\\}
\STATE \For{$i$=1 to $n_{cluster}$} {
$\hat{\counterexSet}_{vec}\leftarrow minimum(\counterexSet_{vec}^i,3,'\rho_{cex}')$
\texttt{/* select cex with smaller robustness values  */} ~\\}
%\STATE $\counterexSet = \counterexSet_m \cup \counterexSet_g$ 
%\texttt{/* collecting all the counterexamples */} ~\\
%\STATE $\dataset_{i+1} =  \dataset_{i} \cup Select_{cex}(\counterexSet) \cup Select_{ex}(\exampleSet)$ 
%\texttt{/* update the data set */}~\\
\STATE $\hat{\counterexSet}_{vec}=Concat(\hat{\counterexSet}_{vec}^i)$ \texttt{/* Concatenating clustered counterexamples */}\\
\STATE $\hat{\counterexSet}= \beta(\hat{\counterexSet}_{vec})$
\texttt{/* Mapping set-points back to traces */}\\
\end{algorithmic}
\caption{Counterexample Selection}
\label{algo:dataextraction}
\end{algorithm}


==> iccps2023_version/conclusion.tex <==
\section{Conclusion}
\label{sec-conclusion}

We have introduced the problem of synthesizing a neural network controller for a nonlinear dynamical system where the specification is given as a set of STL formulas. We have presented a counterexample-guided controller refinement algorithm to solve the synthesis problem.  The algorithm is based on generating initial training data satisfying a coverage criterion and then subsequent retraining based on the training data generated from the counterexamples. Our experimental results demonstrate that the proposed technique is capable of synthesizing NN controllers for non-trivial dynamical systems with a set of complex STL specifications. We have also shown that it is possible to construct a NN that can satisfy a set of properties that may be difficult to satisfy jointly by a single controller using conventional methods.
Finally, our success in synthesizing a NN controller to replace a MPC establishes that our technique is capable of replacing a computationally inefficient but high-performance controller with a computationally efficient NN controller without any degradation in the control performance.

Our experimental results demonstrate that the neural networks need not be too large to become an efficient feedback controller. However, more complex dynamical systems and specifications may demand larger neural networks, making their training challenging.
In our future work, we plan to evaluate the effect of the architectural parameters (number of layers, number of neurons each layer, etc.) on the training efficiency.


%In the future, we plan to extend our framework to synthesize a neural network controller from several nominal controllers, each of which is optimal for a subset of the given specifications. We also plan to apply our technique to synthesize NN-controllers for complex dynamical systems like a quadrotor.  

==> iccps2023_version/evaluation.tex <==
%\section{Implementation and Experimental Results}
\section{Evaluation}
\label{sec:experiment}
Given that our work is tailored towards control systems, we have implemented our code in MATLAB\textsuperscript{\textregistered}/Simulink\textsuperscript{\textregistered}  which is widely used for such applications. Starting from a closed-loop system defined in Simulink and a set of formal specifications, we automatically perform coverage-based data generation, training via the MATLAB\textsuperscript{\textregistered} Deep Learning Toolbox~\cite{deep_learning_toolbox}, falsification via the tool Breach~\cite{breach}, counterexample  selection via clustering, and NN retraining. 

%{\color{blue} 
%Let us consider that we have our simulation engine $\simulator$ (Simulink/MATLAB model) which generates traces for the closed-loop system with the nominal controller be in active. We assume that the simulation engine produces samples according to a user-defined sampling rate (time discretization step) $dt$ and the simulation duration (trace time horizon) is $T$. %In general, this rate can be variable or fixed. 

%We  need to plug in the external inputs to $\simulator$, that is $(r(\cdot), x_0)$ (reference signal and initial conditions). The outputs of $\simulator$ are $(y(\cdot), x(\cdot), u(\cdot))$ (output signal, control input signal, state variable signal). 
%Let us define $n_{t}$ as the number of times we call $\mathcal{S}$. For $i \in [1,n_{t}]$, we get  $\mathcal{S}_{in}^i:=\{r^i(\cdot)$, $x_0^i\}$, $\mathcal{S}_{out}^i:=\{y^i(\cdot), x^i(\cdot), u^i(\cdot)\}$. 

%The next step is to choose the data that are needed for training. We define $\mathcal{D}=\{R, Y, U\}$ where $R:=<r^1(\cdot), r^2(\cdot),\ldots,r^{n_t}(\cdot)>$ and similarly $U$ and $Y$ are defined. This operation can be seen as concatenating the parts we need from $\mathcal{S}_{out}^i$ and $\mathcal{S}_{in}^i$. Once we have $\mathcal{D}$, we can get $\mathcal{D}_k=\{R_k, Y_k, U_k\}$, which corresponds to the data evaluated at discrete time. As mentioned above, in our experiments, we configure the solver of the simulation engine to produce outputs at fixed time points, so $\mathcal{D}_k$= $\mathcal{D}$.

%In order to get the inputs and outputs (targets) of the NN, we need to add memory/delayed blocks to capture the dynamic element of the closed-loop system. The output of the NN is $\mathcal{O}=U_k$ and the input of the NN is $\mathcal{I}=\{<R_k,R_{k-1},\ldots R_{k-p_r}>, <Y_k,Y_{k-1},\ldots Y_{k-p_y}>,<U_{k-1},\ldots U_{k-p_u}>~, <E_k, E_{k-1},\ldots E_{k-p_e}>, <SW_k,\ldots SW_{k-p_{SW}}>\}$ where $p_r$ is the number of previous  reference values we wish to introduce to capture memory, $p_y$ is the number of previous $y$ values, $p_u$ corresponds to past $u$ terms and $E_k=R_k-\tilde{Y}_k$. Note that it is possible that not all outputs $Y$ need to be tracked and compared with the corresponding references. Also, notice that the options of $p_r, p_y, p_u, p_e$ have to be made by the user upon evaluating the structure and the dynamics of the nominal controller(s). Experimental results are required to properly check that the selection is sufficient.  Regarding the terms  $SW, p_{SW}$, we introduce them for the case of switched systems. We have seen that adding the switching signal could enable the NN to generalize better. For example, for time-triggered systems,  $SW$ could correspond to the real (simulation) time, i.e. $SW_k=T_k$ where $T_k=\{<0:dt:T>,\dots, <0:dt:T> \}$.~\\
%}


We have applied our methodology to a variety of case studies. We discuss our methodology applying to four types of examples. We use the first set of examples in Section~\ref{sec:standard} to demonstrate different aspects of our methodology and its scalability on a selection of example controllers and plants of varying complexity. In Section~\ref{sec:switched}, we apply our methodology for learning switched systems. In Section~\ref{sec:propertyCombinations}, we demonstrate that it is possible to learn a single NN controller that combines the best features of two different controllers. Finally, in Section~\ref{sec:mpc}, we demonstrate that our methodology is applicable to learning a NN controller from a Model Predictive Controller, establishing that our methodology is capable of synthesizing a controller with the comparable control performance of a standard high-performance controller while reducing the computational inefficiency significantly.


%We have applied our methodology to two case studies, a water-tank level controller~\cite{watertank} and a robot-arm controller~\cite{robotarm}. Both are closed-loop systems and the nominal controllers are discrete-time PID (one-degree of freedom PID and two-degree of freedom PID respectively). The water-tank has 1 state variable, 1 output variable, 1 reference, and nonlinear dynamics (trigonometric). The robot-arm has 2 state variables, 1 output variable, 1 reference, and nonlinear dynamics (with a square root function). 
%\nk{The continuous stirred reactor tank probably future work} %Figure~\ref{fig:methodology} demonstrates our methodology for retraining. % with the aim to eliminate counterexamples and guarantee that the NN satisfies a set of properties. 
%In our setup, we use the Deep Learning Toolbox from MATLAB to train the neural network, and the tool Breach~\cite{breach} for property checking/falsification tool. We train a NN structure consisting of two hidden layers along with the input and output layers. The inputs to NN consist a subset combining current variables with a limited number of past variables. The hidden layers have 30 neurons each with hyperbolic tangent activation. The output layer is made up of the control variables. 
%\is{Should we interchange the position of Figure 2(a) and 2(b)?}

%In each experiment, we begin with a set of properties representing specifications that the NN model should meet. 

In our experiments we use a combination of four properties: \textit{Matching Error (M)}, \textit{Stabilization (St)}, \textit{Settling time (Se)}, and \textit{Overshoot (O)}, which are expressed in STL, where the notation $x[t]$ refers to the value of signal $x$ at time instance $t$. The placeholder $\simtime$ is the temporal length of simulated behaviours. 
The constant parameter $dt$ is used to express a small time duration. 
%The template for stabilization can be used to express settling time by setting parameters $T_1=T_2=0$, $T_3$ to be the specified settling time, and $T_4$ to be the length of time before the reference changes.

%\vspace{-4pt}
\input{property.tex}
%In each experiment what do we show?
%1. Properties
%2. Show existence of counterexamples after initial training
%3. Importance of using clustering
%4. Importance of using counterexamples for re-training vs random re-training - number of retraining samples should be the same in both cases

%\myworries{We use properties defined in Section~\ref{sec:preliminaries}.}



%We apply our methodology on two case-studies, where the nominal controllers are adapted from Simulink models of a water-tank level controller~\cite{watertank} and a robot-arm controller~\cite{robotarm}. 
\subsection{Demonstrating Method Scalability}\label{sec:standard}
In this section we apply our methodology to a selection of examples, as proof-of-concept, to demonstrate different aspects of the methodology. In all examples, the controller used to generate the training data, the nominal controller or teacher, also satisfies the properties used for NN falsification. This ensures that when the NN violates a property, any counterexamples found can be used to generate a new training data set from the NN's respective nominal controller (the teacher). Hence, during retraining, the nominal controller's behaviour also satisfies the chosen property set. 

% The first example in Table~\ref{table:retraining} includes a water-tank level controller~\cite{watertank} used to illustrate the various aspects of our methodology. 
Table~\ref{table:retraining} shows the results for a water-tank level controller~\cite{watertank}, which is used to illustrate the various aspects of our methodology. 
We provide further examples later to demonstrate how our methodology can be applied to a variety of other controller-plant combinations. The water-tank level controller is part of a closed-loop systems and the nominal controller is a discrete-time PID controller (one-degree of freedom PID). The water-tank has 1 state variable, 1 output variable, 1 reference, and nonlinear dynamics (trigonometric). The water-tank controller should have an overshoot of at most $0.07$, stabilize for $1.5\si{\second}$ within $0.025$ of the reference within $3.5\si{\second}$. The properties use a step-change $\epsilon_r$ of $0.01$.  

The structure of the NN used for the water-tank controller has two hidden layers and the output layer has one output. The hidden layers have hyperbolic tangent activation functions and the output layers linear ones. Each hidden layer has $30$ neurons. %Note that the NNs differ in the number of inputs since the PID controllers have inputs of different dimensions. 
The water-tank takes as input the error $e_k=r_k-y_k$ which is one dimensional. %The robot-arm controller has 2 input variables: $r_k$ and $y_k$ (used to compute setpoint weights). 
Fig~\ref{fig:water-tank:structure} illustrates the NN structure used for the water-tank model.

 
%{\color{red} REVIEW A bit more information about the various components of the Water-Tank and Robot-Arm systems would be helpful.}
%\is{Here we are repeating a few points that have been mentioned in the first paragraph. There is also inconsistency -- 20 neurones vs 30 neurons.}
%The inputs to the two NN control models are as follows:
%\begin{itemize}[noitemsep,topsep=0pt]
%    \item \textbf{Water-Tank:} The current and three past reference matching errors, and the past two control outputs.
%    \item \textbf{Robot-Arm:} The current and three past reference values, the current and past three plant outputs, and the past two control outputs.
%\end{itemize}

%Tabulation of Results
%Model
%Iteration (ID)
%Number of traces tested
%Number of counterexamples (We ignore traces that where nominal has counterexamples also)
%Number of counterexamples removed through re-training
%Number of new counterexamples after re-sampling

% Add the size of the grid (10*10) and absolute vakue is not important
%T is the number of system behavior, maybe replace T by B for behaviors
%
\begin{table*}
{
%\scriptsize
\renewcommand{\arraystretch}{1} % For vertical spacing
\setlength{\tabcolsep}{0.5em} % For horizontal spacing
    \centering
    \begin{tabular}{c c c c c c c c c c c c c c}
        \toprule
         \multirow{3}{*}{\begin{tabular}{c} \textbf{Model}\\
         $[\underline{r},\overline{r}]$
         \end{tabular}} 
         & & & & & \multicolumn{5}{c}{\textbf{\# of counterexamples}} & \multicolumn{3}{c}{\textbf{Runtimes} (sec)} \\ \cmidrule(r){6-10} \cmidrule{11-13}
         & \textbf{ID} & \textbf{Clust.} & \textbf{Spec}& \textbf{i} & \textbf{$n_T$} & \textbf{$n_C$} &         \textbf{$n_{\hat{C}}$} &   \textbf{$n_R$} &
         \textbf{$n_{\tilde{C}}$} & %\multicolumn{3}{c}{\textbf{Time} (sec)} %\\
         %\cmidrule{11-13}
         %& & & & & & & & & &
         $t_{T,C,\hat{C}}$ & $t_R$ & $t_{\tilde{C}}$\\
         \midrule %-------------Next model---------------
         \multirow{14}{*}{\begin{tabular}{c} Water-Tank\\
         $[8,12]$
         \end{tabular}} & 
         \multirow{3}{*}{\begin{tabular}{c} $W_{1,1}$\\
         $[8^2]\langle 0.5 \rangle$
         \end{tabular}} & 
         \multirow{3}{*}{No} & 
         \multirow{3}{*}{$O \land St \land Se$} & 
         0 &--&--&--&64 & -- &-- & --& --\\
         & & & &
         1 & 300 & 262 & \textbf{262} & 324 & \textbf{0} & 469.75 & \textbf{4275}& 494.75
         \\  
         & & & &
         2 & 176 & 0& --&--&--&285.94&--&-- \\ 
         \cmidrule{2-13} %----------Next Instance------------
         & 
         \multirow{3}{*}{\begin{tabular}{c} $W_{1,2}$\\
         $[8^2]\langle 0.5 \rangle$
         \end{tabular}} & 
         \multirow{3}{*}{Yes} & 
         \multirow{3}{*}{$O \land St  \land Se$} & 
         0 & --& --&--& 64 & -- &-- & -- & --\\
         & & & &
         1& 300 & 262 & \textbf{9} & 73 & \textbf{0} & 471.04 & \textbf{429}& 504.35\\ 
         & & & & 
         2 & 176  & 0 &-- &-- &-- &  285.94 &--&--\\
        \cmidrule{2-13} %----------Next Instance------------
         & 
         \multirow{3}{*}{\begin{tabular}{c} $W_{1,3}$\\
         $[8^2]\langle 0.5 \rangle$
         \end{tabular}} & 
         \multirow{3}{*}{Random} & 
         \multirow{3}{*}{$O \land St \land Se$} & 
         0 & --& --&--& 64&--&--&--&--\\
         & & & &
         1& 300 & 262 & \textbf{9} (rand) & 73 & \textbf{60} & 482.71 & 996.74 & 498.66 \\ 
         & & & & 
         2 & 100 & 113$^*$&-- &-- &-- & 183.55 &--&--\\
         \cmidrule{2-13} %----------Next Instance------------
         & 
         \multirow{3}{*}{\begin{tabular}{c} $W_{2}$\\
         $[4^2]\langle 1 \rangle$
         \end{tabular}} & 
         \multirow{3}{*}{Yes} & 
         \multirow{3}{*}{$M \land St$} & 
         0 & --& --&--& 256\\
         & & & &
         1& 100 & 3 & 3 & 259 & 0 & 199.94 & 721.29 & 98.27 \\ %4 new cex from T-\hat{C}
         & & & & 
         2 & 100 &8 & 4 &263 &0 & 195.41 &4161.5&85.7367\\
          & & & & 
         3 & 200 & 0&-- &-- &-- & 404.84 &--&--\\
         %\midrule %-------------Robot Arm model---------------
         %\multirow{11}{*}{Robot-Arm} & 
         %\multirow{3}{*}{\begin{tabular}{c} $A_{1,1}$\\
         % $[3^2]\langle 0.33 \rangle$
         %\end{tabular}} & 
         %\multirow{3}{*}{Yes} & 
         %\multirow{3}{*}{$O$} & 
         %0 & -- & -- & -- & 9 & -- & -- & --& --\\
         %& & & & 
         %1 & 100 & 33 & 8 & \textbf{17} & 0 & 494.7 & 9.48 & 269.87 \\ %8/9
         %&  & & & 
         %2 & 200 & 0&--&--&--&956.79&--&-- \\ 
         %\cmidrule{2-13} %----------Next Instance------------
        %  &
        %  \multirow{4}{*}{
        %  \begin{tabular}{c} $A_{1,2}$\\
        %  %$\langle 0.33 \rangle$
        %  $[3 \times 3]$ $\langle 0.33 \rangle$
        %  \end{tabular}} &         
        %  \multirow{4}{*}{No} & 
        %  \multirow{4}{*}{St} & 
        %  0 & - & - & - & 9 & - & 20.24 & 13.51& -\\
        %  & & & & 
        %  1 & 100 & 74 & 74 & 83 & 28 & 458.44 & 46.81 & 390.36\\ 
        %  &  & & & 
        %  2 & 100 & 32 & 32 & 115 & 31 & 462.74 & 46.08 & 265.48\\
        %  & & & &
        %  3 & 100 & 20 & 20 & 135 & 15/21 & 396.38 & 904.14 & 240.62\\
         %&
         %\multirow{4}{*}{
         %\begin{tabular}{c} $A_{1,2}$\\
         %$\langle 0.33 \rangle$
         %$[3^2]\langle 0.33 \rangle$
         %\end{tabular}} &         
         %\multirow{4}{*}{Yes} & 
         %\multirow{4}{*}{$St$} & 
         %0 & -- & -- & -- & 9 & -- & -- & --& --\\
         %& & & & 
         %1 & 100 & 46 & 12 & 21 & 0 & 476.84 & 15.23 & 280.84\\ %6/29
         %&  & & & 
         %2 & 100 & 36 & 9 & \textbf{30} & 0 & 487.12 & 13.77 & 277.38\\
         %& & & &
         %3 & 200 & 20 & -- & -- & -- & 1029.5 & -- & --\\
        %\cmidrule{2-13} %----------Next Instance------------
        %&
         %\multirow{4}{*}{
         %\begin{tabular}{c} $A_2$\\
         %%$\langle 0.33 \rangle$
         %$[9^2]\langle 0.14 \rangle$
         %\end{tabular}} &         
         %\multirow{4}{*}{No/Yes} & 
         %\multirow{4}{*}{$O \land St \land Se$} & 
         %0 & -- & -- & -- & 47 & -- & -- & --& --\\
         %& & & & 
         %1 & 100 & 1 & 1  &  48& 0 & 535.88 & 21.40 & 263.60\\ 
         %&  & & & 
         %2 & 200  & 3 & 3 & 51 & 0 & 1068.2 &33.54  &283.49 \\
         %& & & &
         %3 & 200 & 0  & -- &--  &--  & 990.65 &--  &-- \\
         \bottomrule\\
    \end{tabular}
    \caption{\small Counterexample (cex) elimination through guided iterative re-training. $\mathit{ID}$: initial training instance of the neural network. $[l^m]\langle\delta\rangle$: Piece-wise constant reference with domain partitioned into $l$ segments, with $m$ time intervals, with minimum separation $\delta$ between reference points.  $i$: retraining iteration. $n_T$: \# of behaviours explored by the falsifier in the iteration. $n_C$: \# of cex identified from $n_T$ behaviours. $n_{\hat{C}}$: \# of cex left after clustering (if clustering is used). 
    %If clustering is used, $n_{\hat{C}}$ is the number of counterexamples left after clustering. 
    $n_R$: \# of behaviours for (re-)training. $n_{\tilde{C}}$: \# of remaining cex after testing on the training data. $t_{XYZ}$: time for computing columns labelled $n_{XYZ}$. { 9 (rand)}: 9 randomly generated traces -- no clustering. *: 60 cex from previous iteration and 53 new cex.} %A2: stopped after 3 iterations \textcolor{red}{To illustrate the point of Goran in the Intro. Overshoot/Transient property was captured with only 9 traces but stabilization was not}
    \label{table:retraining}
}
\end{table*}

%\is{Why are we using different inputs for the two models? Is it possible to provide the justification?}

%\is{We do not provide any details about the nominal controller. This may raise question.} \ab{Added a statement earlier referencing the nominal controllers with a citation to Mathwork pages}

In general, for each NN controller, we generate training data from the nominal controller using coverage metrics discussed in Section~\ref{sec:covData}. Initial training, although coverage-based and exhaustive, may not be sufficient to guarantee a NN's adherence to specifications. The input stimuli for each case study are described by piecewise-constant functions with a varying number of setpoints. We then use our cex guided retraining approach to identify cexs, conduct clustering to select the most representative ones (not necessarily the ones with the worst robustness), retrain the NN, and show that we are able to obtain a NN controller that does not have any closed-loop cex.

%\color{red}

%\subsection{Water Tank}

% Add comparison between cex-guided retraining vs adding random points
\begin{figure*}[t!]
    \centering
	%\hspace{-5em}
	\begin{subfigure}[b]{0.25\textwidth}
	\centering
	    \hspace{0.2em}
	    %\raisebox{+\height/4}{
	    \includegraphics[width=1.0\textwidth]{figures/water-tank/nn.eps}
	    %}
	\caption{\small NN Structure with inputs including error terms $e_k = r_k-\overline{y}_k$, and past control outputs $\overline{u}_{k-1}$, $\overline{u}_{k-2}$.}
	\label{fig:water-tank:structure}
	\end{subfigure}~
	\quad
	\begin{subfigure}[b]{0.7\textwidth}
	    %\hspace{-3.8em}
		%\raisebox{-\height/2}{
		\includegraphics[width=\textwidth,trim={4cm 0 4.1cm 0},clip]{figures/water-tank/watertank_1by9_comp2.eps}
		%}
		\caption{\small Behaviour under reference with eight time intervals.}
		\label{fig:water-tank:longTrace}
	\end{subfigure}
	\caption{\small Water-tank control for tracking a reference water level (red). Plant outputs using the PID controller (black), NN controller before (magenta) and after retraining (blue).}\label{fig:water-tank}
\end{figure*}

Figure~\ref{fig:water-tank:longTrace} shows a cex behaviour for the water-tank system (magenta) observed when using the NN trained initially with the coverage-based generated training data. Beyond the first three reference steps, the original NN is unable to effectively control the plant. This cex along with others are used for retraining. The result of applying our method is a correct-by-specification closed-loop response shown in blue.

Table~\ref{table:retraining} shows the results of re-training on the water-tank controller using a variety of choices of clustering methods and property combinations. Note that we check several properties at the same time and eliminate the cex that correspond to each individual property. The experiments $W_{1,1}$,$W_{1,2}$ $W_{1,3}$ are run with the same configuration. The first round of falsification uses $300$ traces and identifies $262$ cexs. From $W_{1,1}$ and $W_{1,2}$, we observe the importance of clustering. In $W_{1,2}$ clustering selects only 9 cexs, but they are enough to eliminate all 262 cexs. Selecting all cexs for retraining would also eliminate them but at the expense of a $10$ times greater computational time. Comparing $W_{1,2}$ and $W_{1,3}$ highlights the importance of a guided-approach. Selecting $9$ traces at random from the allowed possible ones for retraining is not adequate to eliminate all $262$ cexs. Further, for $W_{1,3}$, in the next iteration, we test with $100$ new traces and we identify $50$ new cexs. In $W_{2}$, there are $4$ setpoints necessitating the need for more traces to guarantee $100\%$ cell occupancy. After $3$ iterations, it is possible for the NN to eliminate all the cexs.

%The experiments $A_{1,1}$ and $A_{1,2}$ are trained using the same training set of piece-wise constant signals having two pieces, chosen from 3 values with a separation of 0.33. However, they differ with respect to the properties used for falsification. Experiment $A_2$ uses a training set with piece-wise constant behaviours having two pieces, with each piece chosen from 9 values separated by 0.14. Additionally, $A_2$ uses three properties for falsification. For $A_2$, the number of cex found during falsification is small, hence clustering has no impact on $n_{\hat{C}}$. $A_{1,1}$ and $A_{1,2}$ indicate our empirical finding that properties that the NN needs more training data to capture properties that relate to the steady state in comparison with properties that correspond to the transient behaviors describe the steady state behavior typically need more training data

%------------New Experiments---------------
We further apply our methodology on other examples of varying types and complexity. The results of counterexample-guided NN training for these are summarized in  Table~\ref{table:additional}. The example systems used therein are described below:
\begin{enumerate}
    \item \textit{Robot Arm~\cite{robotarm}:} 
    The robot-arm controller is part of a closed-loop system having a discrete-time PID with two-degrees of freedom. The controller has 2 state variables, 1 output variable, 1 reference, and nonlinear dynamics (with a square root function). The NN is evaluated using the properties (having common values for $T_{sim}=10$, $\epsilon_r=0.01$) for overshoot ($T_7=0.4$, $T_8=1$, $\epsilon_y=0.1$), settling time ($T_5=3$, $T_6=4$, $e'=0.05$)  and stabilization ($T_1=0$, $T_2=3$, $T_3=0$, $T_4=2$, $e=0.015$) properties. 
    The NN is feedforward with $2$ hidden layers each having $30$ neurons. The NN has $10$ inputs, $r_k$, $r_{k-1}$, $r_{k-2}$, $r_{k-3}$, $y_{k}$, $y_{k-1}$, $y_{k-2}$, $y_{k-3}$, $u_{k-1}$, $u_{k-2}$.
%training_options.use_previous_u=2;
%training_options.use_previous_ref=3;
%training_options.use_previous_y=3;

%training_options.neurons=[30 30];

    \item \textit{Quadcopter~\cite{quadcopter}:} %[Expt 5]
    The controller for translational-position ($x$ and $y$ axes) is implemented as two PID controllers, one for the $x$-axis and one for the $y$-axis. The example demonstrates capturing non-linear control logic for the translational-position PID using the NN.  The NN is evaluated using the stabilization property in the $x$ and $y$ directions ($T_{sim}=50$, $\epsilon_r=0.0001$, $dt=0.01$, $T_1=0$, $T_2=20$, $T_3=0$, $T_4=5$, $e_{1}=0.001$, $e_{2}=0.001$).
The NN is feedforward with $2$ hidden layers each having 30 neurons. The NN has $15$ inputs, $r_k$, $r_{k-1}$, $r_{k-2}$, $y_{k}$, $y_{k-1}$, $y_{k-2}$. Note that $r$ is $2$-dimensional and $y$ is $3$-dimensional.
%phi:= alw_[0,sim_time] ((abs(In1[t+dt]-In1[t])>d or [t]==0) => (ev_[0,T_1] alw_[0,T_2] ((abs(y_2_[t]-In1[t])<e) and (abs(y_3_[t]-In2[t])<e_y))))
    \item \textit{Vehicle engine speed control~\cite{engine}: }%[Expt 7] is based on published results by Crossley and Cook (1991) (\url{https://www.mathworks.com/help/simulink/slref/modeling-engine-timing-using-triggered-subsystems.html}
    The model describes a four-cylinder spark ignition internal combustion engine. The work in Ref.~\cite{engine} also shows how a simulation based on this model was validated against dynamometer test data. The model uses a highly non-linear switched plant having 6 simulink blocks. We show that the single PID controller for the plant can be replaced by a NN. The NN is evaluated using the stabilization property ($\epsilon_r=0.01$, $dt=0.01$, $T_{sim}=30$, $T_1=0$, $T_2 = 7$, $T_3 = 0$, $T_4=8$, $e=0.15$). The NN is feedforward with $2$ hidden layers each having $30$ neurons. The NN has $8$ inputs, $r_k$, $r_{k-1}$, $r_{k-2}$, $r_{k-3}$, $y_{k}$, $y_{k-1}$, $y_{k-2}$, $y_{k-3}$.
\end{enumerate}

\begin{table*}
{
%\scriptsize
\renewcommand{\arraystretch}{1} % For vertical spacing
\setlength{\tabcolsep}{0.5em} % For horizontal spacing
    \centering
    \begin{tabular}{c c c c c c c c c c c}% c c c}
        \toprule
         %& & & 
         & & & \multicolumn{5}{c}{\textbf{\# of counterexamples}} & \multicolumn{3}{c}{\textbf{Runtimes} (sec)} \\ \cmidrule(r){4-8} \cmidrule{9-11}
         \textbf{Model} & \textbf{Desc.} & \textbf{i} & \textbf{$n_T$} & \textbf{$n_C$} &         \textbf{$n_{\hat{C}}$} &   \textbf{$n_R$} &
         \textbf{$n_{\tilde{C}}$} & %\multicolumn{3}{c}{\textbf{Time} (sec)} %\\
         %\cmidrule{11-13}
         %& & & & & & & & & &
         $t_{T,C,\hat{C}}$ & $t_R$ & $t_{\tilde{C}}$\\
         \midrule %-------------Next model---------------
         %-------------Vehicle engine speed control---------------
         \multirow{4}{2cm}{\centering Robot-Arm} & 
         \multirow{4}{*}{\begin{tabular}{c} $[-0.5 ,0.5 ]$\\
         $[7^2]\langle 1/7 \rangle$
         \end{tabular}} &
         0 & -- & -- & -- & 49 & -- & -- & --& --\\
         &  
         &
         1 & 100 & 1 & 1  &  50& 0 & 535.88 & 21.40 & 263.60\\ 
         & 
         &
         2 & 200  & 3 & 3 & 53 & 0 & 1068.2 &33.54  &283.49 \\
         &
         &
         3 & 200 & 0  & -- &--  &--  & 990.65 &--  &-- \\
         \midrule
         %-------------Quadcopter---------------
         %trace_gen: %34.49s -- training: 2023s
         \multirow{4}{2.4cm}{\centering Quadcopter} & 
         \multirow{4}{*}{\begin{tabular}{c} $x\in[0.2,0.4]$\\
         $[30^2]\langle 0.2/30 \rangle$\\
         $y\in[0,0.1]$\\
         $[30^2]\langle 0.1/30 \rangle$
         \end{tabular}} & 0 & -- & -- & -- & 30 & -- & -- & --& --\\
         &
         &
         1 & 100 & 2 & 2 & 32 & 0 & 613.07 & 733 & 358.14 \\ %8/9
         &
         &
         2 & 100 & 13 & 11 & 43 & 0 & 688.98 & 1061.90 & 383.21 \\
         &
         &
         3 & 200 & 0 & -- & -- & -- &1311.12 & -- & --\\
         \midrule
            \multirow{3}{2cm}{\centering Vehicle Engine Speed Control} & 
         \multirow{3}{*}{\begin{tabular}{c} $[2000 ,2050 ]$\\
         $[7^2]\langle 50/7 \rangle$
         \end{tabular}} & 
         0 & -- & -- & -- & 49 & -- & -- & --& --\\
         &
         &
         1 & 100 & 17 & 15 & 64 & 0 & 288.24 & 3130 & 153.18 \\ %8/9
         &
         &
         2 & 200 & 0 & -- & -- & -- & 619.17 & -- & -- \\ 
         \bottomrule\\
    \end{tabular}
    \caption{\small Counterexample (cex) elimination through guided iterative re-training. $\mathit{Desc.}$: Reference interval $[\underline{r},\overline{r}]$,  $[l^m]\langle\delta\rangle$: Piece-wise constant reference with domain partitioned into $l$ segments, with $m$ time intervals, with minimum separation $\delta$ between reference points. For the quadcopter there are two references for the $x$ and $y$ axes, with ranges and grid partitioning for each mentioned separately. $i$: retraining iteration. $n_T$: \# of behaviours explored by the falsifier in the iteration. $n_C$: \# of cex identified from $n_T$ behaviours. $n_{\hat{C}}$: \# of cex left after clustering (if clustering is used). 
    %If clustering is used, $n_{\hat{C}}$ is the number of counterexamples left after clustering. 
    $n_R$: \# of behaviours for (re-)training. $n_{\tilde{C}}$: \# of remaining cex after testing on the training data. $t_{XYZ}$: time for computing columns labelled $n_{XYZ}$.} 
    \label{table:additional}
}
\end{table*}


\subsection{Learning Switched Controllers}\label{sec:switched}
In this section we demonstrate the application of our methodology to learn a single NN that captures the behaviour of a switched controller. We apply the method to three examples, a 3-location switched controller, a gain-scheduled PID controller where the p-i-d terms are defined by a lookup table, and a fuzzy inference system the uses a lookup table in conjunction with a PID controller.

The results of using our methodology on these examples are summarized in Table~\ref{table:switched}. The examples are described below:
\begin{enumerate}
    \item \textit{3-Location Switched Controller~\cite{3-locationSwitched} :} %[Expt 9]
    The plant is linear and 2-dimensional; for the controller y-u-r are one dimensional. The controller is a three-location switched controller, with the three locations being \textit{no-action}, \textit{p controller} - requires less computational effort and less accurate, and a \textit{PID controller}. The combination is learned as a single NN and counterexample learning is performed using the property of stabilization (with $T_1=0$, $T_2=6$, $T_3=0$, $T_4=4$, $T_{sim}=20$, $e=0.01$, $dt=0.01$). The NN has $6$ inputs, $r_k$, $r_{k-1}$, $r_{k-2}$, $y_{k}$, $y_{k-1}$, $y_{k-2}$. 
    
    \item \textit{Continuous Stirred Tank Reactor~\cite{gainScheduled} : } %[Expt 4] 
    Gain-Scheduled PID Controller having 2 dimensions, is highly non-linear, and the p-i-d terms are defined using lookup tables. The controller output $u$, plant output $y$, and reference $ref$ are one-dimensional.  The example demonstrates the methods applicability to replicate the gain-scheduled switching logic and lookup table. The NN is evaluated using the stabilization property  (with $T_{sim}=30$, $T_1=0$, $T_2=7$, $T_3=0$, $T_4=8$, $e=0.1$, $dt=0.01$). The NN is feedforward with $2$ hidden layers each having $30$ neurons. The NN has $8$ inputs, $r_k$, $r_{k-1}$, $r_{k-2}$, $y_{k}$, $y_{k-1}$, $y_{k-2}$, $u_{k-1}$, $u_{k-2}$.
    
    \item \textit{Fuzzy inference system~\cite{fuzzy} : }%[Expt 8] 
    The controller contains a $2$-input, $1$-output, $15 \times 15$ lookup table feeding its output to a PID controller. The lookup table takes inputs as the error between the reference and plant output, and the change of plant output $y_k - y_{k-1}$. The output 
    %is a control output $u$, which 
    of the lookup table is in used by the PID. The plant is $3$-dimensional and linear. Lookup tables may require a lot of memory and large computation time when their size is considerable. 
    %\is{The same is applicable for the NN Controller.}\td{The sentence "Lookup tables can require a lot of memory... " could be changed into: Lookup tables may require large computation time especially when their size is considerable.}
    We replace the lookup table - PID combination using a NN. The NN is evaluated using the stabilization property (with $T_1=0$, $T_2=6$, $T_3=0$, $T_4=4$, $T_{sim}=20$, $e=0.01$, $dt=0.001$). The NN we use is feedforward with 2 hidden layers having 30 neurons each. The NN has $6$ inputs, $r_k$, $r_{k-1}$, $r_{k-2}$, $y_k$, $y_{k-1}$, $y_{k-2}$.
\end{enumerate}


\begin{table*}
{
%\scriptsize
\renewcommand{\arraystretch}{1} % For vertical spacing
\setlength{\tabcolsep}{0.5em} % For horizontal spacing
    \centering
    \begin{tabular}{c c c c c c c c c c c}% c c c}
        \toprule
         %& & & 
         & & & \multicolumn{5}{c}{\textbf{\# of counterexamples}} & \multicolumn{3}{c}{\textbf{Runtimes} (sec)} \\ \cmidrule(r){4-8} \cmidrule{9-11}
         \textbf{Model} & \textbf{Desc.} & \textbf{i} & \textbf{$n_T$} & \textbf{$n_C$} &         \textbf{$n_{\hat{C}}$} &   \textbf{$n_R$} &
         \textbf{$n_{\tilde{C}}$} & %\multicolumn{3}{c}{\textbf{Time} (sec)} %\\
         %\cmidrule{11-13}
         %& & & & & & & & & &
         $t_{T,C,\hat{C}}$ & $t_R$ & $t_{\tilde{C}}$\\
         \midrule %-------------Next model---------------
         %-------------Vehicle engine speed control---------------
         \multirow{5}{2cm}{\centering 3-Location Switched Controller} & 
         \multirow{5}{*}{\begin{tabular}{c} $[0 ,1 ]$\\
         $[5^2]\langle 0.2 \rangle$
         \end{tabular}} & 
         0 & -- & -- & -- & 25 & -- & -- & --& --\\
         & 
         &
         1 & 100 & 22 & 22 & 47 & 0 & 101.61 & 203.61 & 81.15 \\ %8/9
         &
         &
         2 & 100 & 5 & 5 & 52 & 0 & 93.37 & 243.59 & 69.08\\ 
          & 
          &
         3 & 100 & 7 & 7 & 59 & 0 & 89.48 & 638.42 & 66.74\\ 
         &
         &
         4 & 200 & 0 & --& -- & --& 163.34& --& -- \\
        \midrule 
        \multirow{3}{2cm}{\centering Continuous Stirred Tank Reactor} & 
        \multirow{3}{*}{\begin{tabular}{c} $[6,7]$\\
         $[\sqrt{40}^2]\langle 1/\sqrt{40} \rangle$
         \end{tabular}}& 
        0 &--&--&--& 40 & -- &-- & --& --\\
         &
         &
         1 & 100 & 2 & 2 & 42 & 0 & 138.62 & 3456.4 & 72.05
         \\  
         &
         &
         2 & 200 & 0 & -- &-- & -- & 331.89 & -- & -- \\ 
         \midrule
         %-------------Fuzzy Inference---------------
         \multirow{5}{2cm}{\centering Fuzzy inference system [PID + lookup table]} & 
         \multirow{5}{*}{\begin{tabular}{c} $[0 ,2 ]$\\
         $[5^2]\langle 0.4 \rangle$
         \end{tabular}} & 
         0 & -- & -- & -- & 25 & -- & -- & --& --\\
         & 
         &
         1 & 100 & 96 & 73 & 98 & 0 & 206.24 & 94.61 & 126.90 \\ %8/9
         &
         &
         2 & 100 & 1 & 1 & 99 & 0 & 184.62 &86.37&154.53 \\ 
         &
         &
         3 & 100 & 2 & 2 & 101 & 0 & 155.05 & 91.67 & 95.96\\
         &
         &
         4 & 200 & 0 & -- & --& --&323.43 & --&--\\
         \bottomrule\\
    \end{tabular}
    \caption{\small Counterexample (cex) elimination through guided iterative re-training. $\mathit{Desc.}$: Reference interval $[\underline{r},\overline{r}]$,  $[l^m]\langle\delta\rangle$: Piece-wise constant reference with domain partitioned into $l$ segments, with $m$ time intervals, with minimum separation $\delta$ between reference points. $i$: retraining iteration. $n_T$: \# of behaviours explored by the falsifier in the iteration. $n_C$: \# of cex identified from $n_T$ behaviours. $n_{\hat{C}}$: \# of cex left after clustering (if clustering is used). 
    $n_R$: \# of behaviours for (re-)training. $n_{\tilde{C}}$: \# of remaining cex after testing on the training data. $t_{XYZ}$: time for computing columns labelled $n_{XYZ}$.}
    \label{table:switched}
}
\end{table*}


%\subsection{Learning to Satisfy a Combination of Properties}
\subsection{Learning a Combination of Controllers Satisfying Different Properties}
\label{sec:propertyCombinations}
In this section, we demonstrate how our methodology can be used to learn a single NN controller that incorporates the best qualities of two controllers. The NN is taught to satisfy a set of properties that are difficult to satisfy jointly using conventional methods.


Our example is for a water-tank level controller. We use two independent PID controllers ($C_1$ and $C_2$) tuned with different goals. The tank is a one-dimensional non-linear plant. The controller $C_1$ has a rise-time of $0.3\si{\second}$, a settling time of $2.54\si{\second}$, and a small overshoot of $10.1\%$; $C_2$ has a rise-time of $0.11\si{\second}$, a settling time of $0.95\si{\second}$, and a high overshoot of $13.1\%$. 

We express two requirements, a low overshoot (expressed as property $\varphi_1$) and a low settling time (property $\varphi_2$). We have:  $C_1 \models \varphi_1$, $C_1 \not \models \varphi_2$ and $C_2 \models \varphi_2$, $C_2 \not \models \varphi_1$. %$\{C_1, C_2\} \not \models \varphi \wedge \varphi_2$. \is{What does the last condition mean?}
%\ih{I think there is a typo. It should be $\{C_1, C_2\} \not \models \varphi_1 \wedge \varphi_2$}

Using our methodology, the NN controller $N$ is taught to satisfy a combination of properties which the individual controllers fail to satisfy, i.e., $N \models \varphi_1$ $\bigwedge$ $N \models \varphi_2$. The key component in this application is using a method of data-generation for training by switching between the controllers based on the robustness of satisfying the properties of overshoot and settling time. 

\begin{table*}
{
%\scriptsize
\renewcommand{\arraystretch}{1} % For vertical spacing
\setlength{\tabcolsep}{0.5em} % For horizontal spacing
    \centering
    \begin{tabular}{c c c c c c c c c c c c}% c c c}
        \toprule
         %& & & 
         & & & \multicolumn{5}{c}{\textbf{\# of counterexamples}} & \multicolumn{3}{c}{\textbf{Runtimes} (sec)} \\ \cmidrule(r){4-8} \cmidrule{9-11}
         \textbf{Model} & \textbf{Desc.} & \textbf{i} & \textbf{$n_T$} & \textbf{$n_C$} &         \textbf{$n_{\hat{C}}$} &   \textbf{$n_R$} &
         \textbf{$n_{\tilde{C}}$} & %\multicolumn{3}{c}{\textbf{Time} (sec)} %\\
         %\cmidrule{11-13}
         %& & & & & & & & & &
         $t_{T,C,\hat{C}}$ & $t_R$ & $t_{\tilde{C}}$ \\
         \midrule %-------------Next model---------------
         %-------------Vehicle engine speed control---------------
         \multirow{5}{2.5cm}{\centering Water Tank Control
         (Combining Properties of Two Controllers)} & 
         \multirow{5}{*}{\begin{tabular}{c} $[8,12]$\\
         $[4^2]\langle 1 \rangle$
         \end{tabular}} & 
         0 & -- & -- & -- & 16 & -- & -- & --& --\\
         & 
         &
         1 & 100 & \textbf{5} & 4 & 21 & 0 & 141.36 & 77.56 & 62.34 \\ %8/9
         &
         &
         2 & 100 & \textbf{3} & 3 & 24 & 0 & 88.72 & 470.41 & 67.82  \\
         &
         &
         3 & 100 & \textbf{1} & 1 & 25 & 0 & 77.42 & 161.02 & 64.89 \\
         &
         &
         4 & 200 & 0 & -- & -- & -- & 158.8 & --&-- \\
         \bottomrule\\
    \end{tabular}
    \caption{\small Counterexample (cex) elimination through guided iterative re-training. $\mathit{Desc.}$: Reference interval $[\underline{r},\overline{r}]$,  $[l^m]\langle\delta\rangle$: Piece-wise constant reference with domain partitioned into $l$ segments, with $m$ time intervals, with minimum separation $\delta$ between reference points. $i$: retraining iteration. $n_T$: \# of behaviours explored by the falsifier in the iteration. $n_C$: \# of cex identified from $n_T$ behaviours. $n_{\hat{C}}$: \# of cex left after clustering (if clustering is used). 
    $n_R$: \# of behaviours for (re-)training. $n_{\tilde{C}}$: \# of remaining cex after testing on the training data. $t_{XYZ}$: time for computing columns labelled $n_{XYZ}$. }
    \label{table:propertyCombinations}
}
\end{table*}

In order to construct the neural network, the first step is to generate data/ traces for training. The traces (used for training) must have the desired characteristics, modeling properties $\varphi_1$ and $\varphi_2$. The way this is achieved is as follows: (1) We break the time horizon into time segments of a suitable length $\tau_s$ for the controller switching, taking into consideration the horizon of the STL formula (e.g., the segment length should be at least as large as the horizon of the STL formula in question), %\is{What is the horizon length of an STL formula? Have we defined it?} 
(2) For each timed segment, we evaluate the robustness of each controller starting from exactly the same conditions (configuration, simstate, %\is{What is simstate?},
initial conditions). Specifically, we evaluate the robustness of the conjunction of the properties for $C_1$  and $C_2$. The control response corresponding to the best robustness in that time step is chosen. (3) For stabilization properties,  $\tau_s$ is chosen to be equal to the duration between two reference changes, meaning that once we have a reference change, we also evaluate the controllers for the past segment. Simply put, whenever a reference changes, the controller can also change based on the robustness. Note that we treat each time segment as left closed and right open. (4) The trace segments (corresponding to each time segment) are stitched together and the trace is checked against $\varphi_1 \wedge \varphi_2$. A trace is kept (and used for training) if it satisfies the two properties and otherwise discarded. 

In this manner a set of traces is generated and used to train the neural network. Once the neural network is trained, the falsification tool is used to examine it, and if counterexamples are found, the same trace generation method described above, in accordance with the proposed methodology, is used to construct training data to eliminate the counterexamples.

The result of applying our methodology to this example is summarized in Table~\ref{table:propertyCombinations}. The NN we use is feedforward with $2$ hidden layers having $40$ neurons and 20 neurons respectively. The NN has 6 inputs, $e_k$, $e_{k-1}$, $e_{k-2}$, $e_{k-3}$, $u_{k-1}$, $u_{k-2}$.


\subsection{Learning a Model Predictive Controller (MPC)}
\label{sec:mpc}
In this section, we present the results of application of our approach to learn a neural network controller which can be safely used in place of a MPC. A MPC solves an optimization problem at each time step when the controller is invoked, which requires significant online computation to be carried out on a high-performance and energy consuming processor. On the other hand, a NN controller involves simple arithmetic computations, thus can be implemented on low-cost, energy efficient processors.

We use an example from Mathworks which shows the training, validation, and testing of a deep neural network to imitate an MPC controller~\cite{imLkaMpc}. 
%% Paragraph about the plant and the controller
In this example, there is a car equipped with 
%sensors to measure lateral deviation, relative yaw angle (between the car and the centre of the road), the current lane curvature, and the curvature derivative. 
%The car is equipped with 
a \emph{Lane Keep Assist system} which adjusts the steering angle to keep the car close to the centre of the road. The Lane Keep Assist system employs a MPC. 
%The plant $y$ is linear and it has 4-dimensions. 
The plant  is linear and its output $y$ has $4$-dimensions.
There is one control output $u$, 
%four reference signals captured in $r$, 
and a disturbance signal $\nu$ representing the curvature of the road.
%which affects all state variables. 
The closed-loop system is evaluated via a disturbance rejection property that is encoded as a target reachability property, i.e.,
$(\Box_{[T_1,T_2]}(|\overline{y_1}[t]|<\epsilon_1) \wedge (|\overline{y_2}[t]|<\epsilon_2 ))$ 
%$(\Box_{[T_1,T_2]}(|\overline{y_1}[t] - r_1[t]|<\epsilon_1) \wedge (|\overline{y_2}[t]-r_2[t]|<\epsilon_2 ))$ 
with $T_1=2.3\si{\second}$, $T_2=T_{sim}=3\si{\second}$, $\epsilon_1=0.6$, and $\epsilon_2=0.55$.
% \wedge$
Here, $\overline{y_1}$ represents the lateral velocity of the car and $\overline{y_2}$ lateral deviation between the car and the centre of the road.

%% results of our experiment on top of that
For the neural network, we keep the architecture used by Mathworks, that is a $3$-layer network having $45$ neurons in each layer. The NN has $6$ inputs, $y_k$, $u_{k-1}$, and $\nu_k$. Note that the training done by Mathworks uses random sampling and only considers points (one-step ahead computations) as training data instead of traces. However, this results to a closed-loop system that violates the above STL property
and retraining either with points or with traces cannot eliminate the counterexamples.

On the contrary, employing our proposed methodology can eliminate all the counterexamples. We start by generating data for training based on our coverage-based technique as discussed in Sec.~\ref{sec:covData}. We need to split a $6$-dimensional space with $100\%$ coverage given certain resolutions and run (one-step ahead) simulations based on these points. Specifically, $y_{1_0} \in [-2,2]\langle 0.5\rangle$, $y_{2_0} \in [-1.04,1.04]\langle 0.52\rangle$, $y_{3_0} \in [-1,1]\langle0.25\rangle$, $y_{4_0} \in [-0.8,0.8]\langle0.4\rangle$, $u_0\in [-1.04, 1.04]\langle0.52\rangle$, $\dis_0 \in [-0.15,0.15]\langle0.075\rangle$. The values inside $\langle\rangle$ provide the resolutions in a given dimension. We perform training on these data, followed by the execution of the falsification-retraining loop. For retraining, it is necessary to employ the entire simulation traces to capture the history and the underlying behaviors.

%% more details about the results like number of initial training examples. No. of counterexamples initially. No. of counterexamples after first iteration
Our initial training data included $16,384$ data points. We use $300$ random traces for falsification. In the first iteration of falsification, we find $100$ counterexamples. We retrain the neural network using these counterexamples. We keep all the generated counterexamples as it was important to find the right balance between these (trace-based counterexamples and the original (point-based) training data. Subsequently, we find that all the counterexamples were eliminated. In the next iteration of falsification, we again use $300$ random traces (different ones) and no new counterexample is found. The generation of each  simulation trace (MPC, NN) takes around $0.25\si{\second}$ for an horizon of $3\si{\second}$ and a time step of $0.1\si{\second}$; training and retraining takes $2\si{\minute}$ and $3\si{\minute}$, respectively.

==> iccps2023_version/hscc-2022-reviews.tex <==
SUBMISSION: 67
TITLE: Counterexample Guided Training of Neural Network Feedback Controllers

-------------------------  METAREVIEW  ------------------------
The reviewers appreciate the authors' effort in clarifying some critical concerns
about the paper. Although the paper addresses an exciting and vital problem,
reviewers agree that the authors should explain the contribution of their approach
by closely comparing and discussing with existing works. In addition, soundness is
essential for safe training/repairing neural networks or neural network control
systems, which can not be guaranteed with the proposed technique. Ignoring soundness
in retraining and assuming that the original controller can be used to generate safe
data makes the research problem less challenging.



----------------------- REVIEW 1 ---------------------
SUBMISSION: 67
TITLE: Counterexample Guided Training of Neural Network Feedback Controllers
AUTHORS: Antonio Bruto Da Costa, Thao Dang, Goran Frehse, Inzemamul Haque, Nikolaos
Kekatos, Akshay Mambakam and Indranil Saha

----------- Overall evaluation -----------
SCORE: 0 (borderline paper)
----- TEXT:
This paper presents a counterexample-guided method for training neural network
controllers to imitate an ensemble of "expert" nominal controllers, with the
requirement that the learned controller should (when run in closed-loop with the
plant) satisfy an STL specification. The specific novelty of this paper appears to
be in their use of clustering to select counterexamples that are both diverse (i.e.
well-spaced) and informative (i.e. in regions where the learned controller performs
poorly).

The paper is clear and flows well. The experimental section in particular does a
good job of explaining why the experiments were chosen to highlight different
capabilities of the proposed system. The water tank example in Section 5.1 is
informative, and it clearly demonstrates the benefit of using clustering to select
good counterexamples.

The main flaw of this paper is that its discussion of related work is not sufficient
to allow the reader to understand what the specific contributions of this work are
(in terms of advancing the state of the art). The paper provides a long list of very
general citations for supervised learning, reinforcement learning, and verification
of neural network controllers in settings that are not relevant to the problem at
hand. In contrast, the paper provides relatively few references about the much more
relevant areas of imitation learning (which has many papers on learning from expert
demonstrations) and counterexample-guided inductive synthesis. This is not the first
time STL has been used in control synthesis (see Raman et al, "Reactive Synthesis
from Signal Temporal Logic Specifications" for a receding-horizon controller using
STL, or Leung, Arechiga, and Pavone, "Back-propagation through signal temporal logic
specifications" for a learning-based approach), nor the first time !
 STL has been used in generating counterexamples to guide learning (e.g.
https://arxiv.org/abs/2006.04260v2). Without a more thorough discussion of related
work, it is hard to tell where the specific contribution lies.

In the current state, where the main contribution appears (to me) to be the use of
clustering to find informative counterexamples, I believe that this paper is
borderline. If the authors revise their related work to be more focused and provide
more details about their clustering method, I would upgrade this paper to a weak
accept. If the authors can revise their related work to show that they close a clear
technical gap in (for example) learning from multiple experts or in providing
significant theoretical guarantees on the algorithm (i.e. explicit non-asymptotic
error bounds), then I would consider increasing my rating to a strong accept.

Some additional questions/comments are included below.

- You train on a simple MSE loss; would it be helpful to include the robustness
metric for the desired STL formula directly in the loss? See Leung, Arechiga, and
Pavone "Back-propagation through signal temporal logic specifications".
- Please comment on the computational complexity of constructing an \epsilon-net of
possible controller settings. How many example trajectories are required? How does a
dataset with exhaustive coverage compare with a randomly sampled dataset (e.g. using
generalization error bounds from statistical learning theory)?
- What happens when the expert controllers do not satisfy the STL specification? You
say that an advantage of the NN is that it can learn from controllers that perform
better in different regimes, but you do not provide a mechanism of weighting
controllers according to their performance. Could the learned controller ever
improve on the nominal controllers (more than just combining the best of multiple
controllers)? Or is this outside the scope of the current work? If you make the
assumption that the experts (or at least one expert) satisfies the STL
specification, you should make that clear in your problem statement.
- In the experiments section, more plots would have been helpful, especially to
understand how your method learns better control input than either of its experts in
Section 5.3.
- Regarding one of your conclusions: it is not surprising that good control
performance can be achieved with small networks. The network sizes you cite are in
line with what I consider standard for control problems.



----------------------- REVIEW 2 ---------------------
SUBMISSION: 67
TITLE: Counterexample Guided Training of Neural Network Feedback Controllers
AUTHORS: Antonio Bruto Da Costa, Thao Dang, Goran Frehse, Inzemamul Haque, Nikolaos
Kekatos, Akshay Mambakam and Indranil Saha

----------- Overall evaluation -----------
SCORE: -1 (weak reject)
----- TEXT:
This paper proposes a counter-example-guided approach to synthesize a neural network
controller for a nonlinear dynamical system so that the closed-loop system satisfies
a set of STL specifications. There are two main steps of this approach. First, the
authors sample the system and find counterexamples using Breach. Then, they combine
the examples and counterexamples found in the first step to generate a new training
data set to retrain the network. The applicability of the proposed approach has been
shown via several benchmarks available in Matlab.  

In general, the paper addresses an exciting and meaningful problem. It is
well-written and organized. The evaluation of the proposed approach is thorough.
However, I am concerned about the paper's main technical contributions. In my
opinion, the contribution of this research is not strong enough to be accepted. This
research assumes that the original systems with nominal controllers satisfy the STL
specifications. This assumption eases the proposed retraining process significantly
as finding counterexamples from simulation traces can be done efficiently using
Breach. The authors can easily generate new training data from the original system
with the nominal controller from counterexamples found in the neural network control
system. The neural network controller can be retrained straightforwardly with the
new training data. I do not see any challenges in doing that.  

Please find below some specific questions and comments. 
1) The clustering technique does not help much in the retraining process in most
cases, as the new training data will use most of the counterexamples. Could you
please explain why?
2) What are the initial states of the systems used in the simulation to generate
data for retraining? I see only in the paper that the reference interval is
partitioned to generate data for training neural networks.
3) How do the authors determine how many past reference inputs, outputs, and
control, for example, r[k], r[k-1], r[k-2], r[k-3], y[k], y[k-1], y[k-2] ....  need
to be used for training a neural network?



----------------------- REVIEW 3 ---------------------
SUBMISSION: 67
TITLE: Counterexample Guided Training of Neural Network Feedback Controllers
AUTHORS: Antonio Bruto Da Costa, Thao Dang, Goran Frehse, Inzemamul Haque, Nikolaos
Kekatos, Akshay Mambakam and Indranil Saha

----------- Overall evaluation -----------
SCORE: 2 (accept)
----- TEXT:
Overview:
In this work, the authors introduce a novel approach for retraining neural network
(NN) controllers to satisfy signal temporal logic (STL) specifications. Using the
MATLAB falsification tool Breach, they identify counterexamples where the nominally
trained NN controller violates the STL property. After identifying these
counterexamples, they generate new traces that target correcting the counterexamples
and retrain the NN controller on the new examples as well as a mix of the old. They
demonstrate their approach on 8 different examples, showing their approach
consistently produces trained NN controllers that Breach is unable to compute any
counterexamples for.
        
Strengths:
- The problem and solution are both well defined and formulated, and the problem is
important and interesting
- Lots of examples provided as case studies demonstrates usability on more than just
one problem

Weaknesses:
- There are existing papers where the authors train NN controllers to satisfy STL
specifications using RL as the training method, [3,4], which appears similar to the
approach of this paper.
- The authors define Properties 1-4 with important metrics for analyzing the NN
controller. It would be good to show the min and max of those properties evaluated
on a large number of generated traces. That might show the improvements provided by
NN controllers over the nominal PID. Figure 2 was an attempt at doing this, but it
shows a single trace which isn't enough to show improvement.
- Authors mention how closest work (Claviere et al.) is limited to memoryless
controllers and their approach is not. However, none of the examples require memory;
all are feedforward NN.

Minor comments:
- The training method used is Behavior Cloning [1] but is left unmentioned
- Should reference some more similar retraining approaches that focus on property
satisfaction ([2] is one example, but there are lots more)
- The authors keep using "counterexample (cex)" but almost never use "cex" on it's
own. Might want to consider removing "cex"
- Algorithm 1 extends beyond the border at lines 528-530
- Line 829 has "in Ref. [45]" but previously the notation has been "in [#]"
- Inconsistencies in the references. Some have author names written out (e.g. John
Doe) while other have initials (e.g. J. Doe). 
- The authors may be interested in the ARCH-COMP AINNCS category benchmarks held the
past few years, and likewise, the case studies of this paper may be of interest for
that category, see e.g.: https://easychair.org/publications/paper/Jq4h

Questions:
- Most examples are already solved by PID. How is using a NN better in these cases?
PID is computationally efficient (probably more so than a deep NN). More MPC
examples that provide data showing the improved performance of the NN controllers
would be helpful. 
- Synthesizing a NN controller that satisfies STL specifications has already been
introduced [4]. They claim their approach is an improvement to their cited most
similar work (Claviere et al.), but don't include examples that Claviere et al.'s
work can't handle. What are the improvements over this existing work?

References:
[1] D. A. Pomerleau, “Efficient training of artificial neural networks for
autonomous navigation,” Neural computation, vol. 3, no. 1, pp. 88–97, 1991
[2] PHAN, D. T., GROSU, R., JANSEN, N., PAOLETTI, N., SMOLKA, S. A., AND STOLLER, S.
D. Neural simplex architecture. In NASA Formal Methods Symposium (2020), Springer,
pp. 97–114.
[3] JOTHIMURUGAN, K., ALUR, R., AND BASTANI, O. A composable specification language
for reinforcement learning tasks. In Advances in Neural Information Processing
Systems 32, 2019, pp. 13041–13051.
[4] Balakrishnan, A., Deshmukh, J.V.: Structured reward shaping using signal
temporal logic specifications. In: 2019 IEEE/RSJ International Conference on
Intelligent Robots and Systems (IROS). pp. 3481–3486. IEEE (2019)

Post response update:

Thank you for the response to the reviewers' concerns. Given the focusing of the
work within the HSCC community, there are some good contributions in this paper. I
would strongly encourage given the domain the authors do check out the benchmarks
from the AINNCS category at ARCH-COMP and related community efforts, given the
relationship to the class of systems considered, albeit aspects of course are
different (no STL specs as of yet, etc.).



----------------------- REVIEW 4 ---------------------
SUBMISSION: 67
TITLE: Counterexample Guided Training of Neural Network Feedback Controllers
AUTHORS: Antonio Bruto Da Costa, Thao Dang, Goran Frehse, Inzemamul Haque, Nikolaos
Kekatos, Akshay Mambakam and Indranil Saha

----------- Overall evaluation -----------
SCORE: -1 (weak reject)
----- TEXT:
This paper presents a method to learn neural network approximations of
several kinds of feedback controllers, using a method based on
coverage-based data generation, then retraining based on generating
counterexamples with a falsifier and clustering them. The evaluation
is comprehensive, spanning several basic feedback controllers,
switched controllers, combination of controllers and even an MPC.

The paper is interesting and well-written, and the results seem
impressive, with an extensive evaluation on a large set of example
controllers.

However, I have two significant concerns about the paper, both
concerning claims from the authors that seem somewhat unsubstantiated,
summarized in the sentence "under some assumptions [...], it is
possible to guarantee that the algorithm always terminates with a
correct NN controller" (line 402). I would be glad to hear the
authors' response on those concerns.

First, you argue that your algorithm always terminates, and you make
this argument more precise in Proposition 2 (line 561). However,
Proposition 2 only refers to being able to retrain with and eliminate
a new counterexample (or maybe a set of them, I'm not so sure). So
what you are actually proving is much weaker: it is saying that you
are able to eliminate one round of counterexamples. But what if you
need several rounds? As in, you have a first set of counterexamples
that you retrain with. But the retrained controller still has a set of
counterexamples that you retrain with. But that new controller still
has a set of counterexamples, etc. You never prove that that process
actually finishes, even though your sentence on line 402 makes it
sound that you do. Worse, a first set of counterexamples might
(theoretically) lead to one controller, which can be breached and
retraining leads back to the first controller, leading to an infinite
loop. Why can this not happen? By the way, did that sort of thing ever
happen when computing your examples?

On a related note, I was not able to understand the argument in the
proof of Proposition 2, and clarify whether it also applied to
eliminating a set of counterexamples (rather than one counterexample);
it is disturbing that the set d_{\gamma_s} doesn't even show up in the
proof.

Second, you deem their final controller "safe", which I take as
meaning that the final controller satisfies the STL
specification. However, the method only uses a falsifier (essentially
a fuzzer for controllers) such as Breach, and the controller is deemed
safe by the authors when the falsifier does not find any
counterexample. The problem is that (as far as I understand) such a
falsifier is not sound: if the falsifier cannot find any any
counterexample, it does not mean that there does not exist any
counterexamples. Why then do you claim your final controller is
"safe", and in what sense precisely?

What are the limitations of your approach and what did not work? A
number of things seem to have worked really well, but I would really
like to know what did not work, or what it took to make your examples
work (i.e., first failed experiments, and how you fixed them).

Even though the evaluation is extensive, I was very disappointed to
see that "the controller used to generate the training data, the
nominal controller or teacher, also satisfies the properties used for
NN falsification." Then what's the point of all this, why not just use
the nominal controller (that you need for training data anyway)? I
would abolutely like to see some evaluations where the nominal
controller did not satisfy the specification, and see how the method
performs on those.

As mentioned in 5.1, clustering is really important in the
approach. However, clustering only occupies about 10 lines of the
paper (lines 550-560), leaving out many essential details. I believe
this is so essential it should probably occupy a subsection, or
something close to a subsection. I urge you to provide more details in
your response and especially in the next version of the paper.

Each of your examples seem to have a different number of layers or
neurons per layers. How did you pick those numbers?

In 3.2, you mention only finite-time traces, but then your interval in
the STL formulas can go to infinity. Isn't this at odds, at least
intuitively? Could you clarify?


==> iccps2023_version/impact.tex <==
\section*{Broader Impact}
% Neural network controllers are slowly being established as an alternative of traditional controllers due to their superior computational performance, less hardware requirement and the capability of approximating any nonlinear function precisely. 
Traditionally, deep neural networks have been applied to solving problems such as computer vision, speech recognition, natural language processing, etc., which are not safety-critical.  However, deep neural networks have the potential to be applied to safety-critical cyber-physical systems (CPSs) in the form of a feedback controller. The potential applications include but not limited to autonomous vehicles, intelligent medical devices, smart grids, smart factories, etc. Unfortunately, despite their vast potential, AI-based controllers have not been widely adopted in the industry due to the lack of guarantees on their behavior. 
Our paper paves the way for synthesizing neural network feedback controllers for safety-critical systems with various reliability guarantees. 
We demonstrate that unlike the traditional controllers, it is possible to synthesize a neural network controller that ensures the satisfiability of a wide range of safety and performance requirements for cyber-physical systems.

Though our technique is capable of enhancing the reliability of AI-based CPSs, we should keep in mind that the controller synthesized by our method is not ``correct'' in the absolute sense. Our technique only ensures reliability with respect to a set of specifications. The system is not guaranteed to satisfy any other requirement that we do not consider at the time of synthesis. 
Nonetheless, our controller synthesis technology is expected to bring more confidence to AI-based safety-critical CPSs. We hope to see many novel safety-critical CPS applications that would not have been possible without AI-based solutions.

==> iccps2023_version/intro.tex <==
\section{Introduction}
%
Neural networks (NNs) have  long been used to control dynamical systems from inverted pendulums to quadcopters, %\cite{citations?}, 
learning from scratch to control the plant by maximizing an expected reward, e.g.~\cite{hagan2002introduction,Nicol08}. %\ih{citations have to be provided here}
NNs can also be trained to replace an existing controller that is unsatisfactory for non-functional reasons, e.g., computationally expensive (consider model-predictive control~\cite{mpc}), slow, or energy intensive. %\cite{cite Indranil MPC?}.
A well-trained NN controller can provide the same performance much faster and is readily implemented on cheap and energy-efficient embedded platforms~\cite{varshney2019deepcontrol}.
We assume that a controller is available and that we can use it to drive the plant (or a model of the plant), observing its inputs and outputs. 
%Our goal is to train a NN that behaves the same as the nominal controller and possibly achieves better performance. 
%\is{This sentence needs modification.}
Our goal is to train a NN that learns from examples generated by some nominal controllers and possibly combines their qualities to achieve better performance globally.
Our approach is characterised by three key features: (i) we observe the nominal controller in closed-loop with the plant, 
%we can train NN controllers to satisfy complex temporal properties, 
%\is{revisit this point.} 
(ii) the training of NN controllers are guided by closed-loop complex temporal properties, and (iii) we leverage the power of existing falsification tools to create training data that matter. In the following paragraphs, we will elaborate these steps.
%

% Training a NN to behave like a nominal controller may look, at first glance, like a simple problem of approximating a function -- the nominal controller -- with a NN.
% One could observe the output of the controller on a dense enough sampling of the input space and use the input-output pairs as training data for the NN.
% In practice, however, there are several difficulties that can be addressed by observing the nominal controller in closed-loop, e.g., while running the plant: 
% \is{Revisit this line.}\td{I suggest to rewrite this paragraph as follows:
Training a NN to behave like a nominal controller is more complex than a problem of approximating a function using pairs of input and output values, since controllers can themselves be stateful dynamical systems. We identify the following difficulties in data generation by executing the nominal controller in closed-loop:
%
\begin{itemize}[noitemsep,topsep=0pt]
    \item 
    \emph{Large input space:} 
    %The number of samples required to cover the input space with sufficient density may be prohibitively large. \td{Change this sentence to: 
    The input space is not only large but can also be infinite. It is thus important to define a coverage measure on the input space to quantify how representative the generated training data is.
    \item \emph{Stateful controller:} When the controller has memory, we need to sample not individual input vectors but its input history. The sampling space increases exponentially with the length of the required history. % GF (the following may be nonsense) : Without the plant, it may be difficult to know how far back one needs to look.
    \item \emph{Non-uniform accuracy:} Depending on the controller specification, the NN may need to be very precise around some inputs while in other input regions a rough approximation is acceptable. 
\end{itemize}
%
% Since a stable controller brings the plant very quickly back to a small neighborhood around its equilibrium or reference trajectory, it suffices to learn in those subspaces. \is{This statement is questionable.}\td{I agree that this is not true in general. We can safely remove this sentence and the one that follows. They do not impact the contents of the paper, since in this paper we do not learn in some particular subspaces.}
% This is easily achieved by observing closed-loop behaviors, which drastically reduces the space to be sampled.\td{as mentioned, I suggest that we remove this sentence.}
%
%
The problem of non-uniform accuracy is particularly pronounced when the specification depends on time or sequences of events. This is frequently the case in control applications, where properties such as \emph{rise time}, \emph{settling time}, and \emph{overshoot} are typical. We consider complex properties that can include not only time but also causal relationships. They can be described in \emph{Signal Temporal Logic} (STL), a formal language that finds widespread use in formal methods and increasing adoption in industry \cite{bartocci2018specification,nickovic2007amt}.
%

While observing closed-loop behaviors may reduce the number of inputs to be sampled, we still need to find good training samples. This problem is not trivial, since uniform sampling turns out to lead to unsatisfactory results, in particular around steady state behaviors, unless very high density is used. %\gf{Can we illustrate this point with a plot of one of our controllers that didn't work?}
In addition, we need to choose the initial state from which to drive the plant, as well as the reference trajectory.
% \is{Isn't this sentence contradicting this line: ``Since a stable controller brings the plant very quickly back to a small neighborhood around its equilibrium or reference trajectory, it suffices to learn in those subspaces.''?}\td{Agreed. The earlier paragraph should be removed.}
%
%
To generate samples that are relevant to the STL properties that we want to satisfy, we leverage existing, highly optimized, \emph{falsification tools} (falsifiers) \cite{annpureddy2011s,breach}. The goal in falsification is to find a \emph{counterexample} (cex), i.e., an input (here, the reference trajectory) and an initial plant state such that closed-loop behavior violates the given STL property. We feed our NN controller, the plant, and the specification to a falsification tool. If the falsifier does not find a cex, we consider our NN controller satisfactory and stop. If the falsifier finds a counterexample, we replay it with the nominal controller in order to obtain new training data, and retrain the network.

%\is{We need to provide a brief description of what we achieve in terms of experimental results.}

In summary, we make the following contributions in this paper:
\begin{itemize}[noitemsep,topsep=0pt]
\item We introduce the problem of synthesising a neural network controller for a nonlinear dynamical system where the specification is given in terms of a set of STL formulas.
\item We provide a counterexample guided controller refinement algorithm to solve the synthesis problem.  Our algorithm is based on generating initial training data satisfying a coverage criterion and then subsequent retraining based on the training data generated from the counterexamples.
\item We implement our algorithm in MATLAB\textsuperscript{\textregistered} using the falsification tool Breach~\cite{breach}. Using our implementation, we successfully synthesise neural network controllers for a variety of example systems satisfying several interesting STL properties.
% \item We demonstrate that it is possible to develop a single NN controller for controllers that have switching or use lookup tables.
% \item We demonstrate that it is possible to train a NN to satisfy a set of properties that may be difficult to satisfy jointly by a single controller using conventional methods.
\item 
%\td{I suggest that we replace the above two items by this one: 
We demonstrate that it is possible to develop a single NN controller that not only can learn from complex controllers (such as those that exhibit switching dynamics or use lookup tables or model-predictive controllers), but also can satisfy a set of properties that may be difficult to satisfy jointly by a single conventional controller.

% \is{The challenges indicated in the last two points could be discussed before where we are discussing the challenges.}
\end{itemize}
%\ih{We need to add that our NN controllers can work as combination of two controllers having different properties.}

%\textcolor{red}{Tone down clustering. One example..  Keep blue part but delete notation.}

==> iccps2023_version/note.tex <==
Date: 19.05.2020

Generally $U$ is used to denote the set of control inputs.

Is it not that a controller is designed to deal with many control settings? Is the notion of region of attraction apt here?

The notion of plant $P$ has not been introduced before Step 1.1.

What is $K$?

In Step 1.1: The control value computed by the set $\mathcal{C}$ of nominal controllers -- The notion of control value computed by a set of controllers is not clear. 



Date: 31.05.2020

$w$ is generally used to denote disturbance in the control literature. Could we use $r$ to denote the reference trajectory?

Date: 02.06.2020

$f((t))$

We may need to provide more intuitive details about the temporal operators. The audience in this conference may not be familiar with temporal logic and may complain that our paper is not fit for the conference.

==> iccps2023_version/problem.tex <==
\section{Controller Learning Problem}
\label{sec-problem}
In this section, we will present the feedback controller learning problem formally.

\subsection{Dynamical Systems and Feedback Controllers}
We consider a continuous-time plant $\Pi$ with state $x \in \reals^n$ that is controlled by an input signal $u$, observed through an output signal $y$, and disturbed by an external signal $\dis$ with dynamics
\begin{eqnarray}
\dot{x}(t)  &=&  f(x(t), u(t), \dis(t)), \label{eq:1}\\
y(t) & = & \zeta(x(t))\nonumber.
\end{eqnarray}
%\is{For the MPC model, we need to introduce disturbance in this equation.}
%\nk{d}
%where $u$ is the control input and $y$ is the plant output. 
The control input $u$ is computed by 
a \emph{nominal} discrete-time controller $\mathcal{C}$ with state $z \in \reals^{n_z}$ %\ih{what is $n_z$ here? Do we need to define it?}
\begin{eqnarray}\label{eq:controller}
z_{k+1} &= & f_c(z_k, y_k, r_k), \\
u_k &= & \upsilon(z_k, y_k,r_k)
\end{eqnarray}
where $r_k$ and $y_k$ are discrete-time signals resulting from sampling the reference $r(\cdot)$ and the output $y(\cdot)$ with a constant time step $\timestep$, that is $\forall k = 0, 1, 2, \ldots, r_k = u(k\timestep), y_k = y(k\timestep)$. The continuous-time control $u(\cdot)$ is a piece-wise constant function defined as $\forall t \in$ $[k\timestep, (k+1)\timestep)~ u(t) = u_k$ with $k = 0, 1, \ldots$. Starting from an initial state $x(0)=x_0 \in X_0$, the behaviour of the system is a vector of functions $\traj=(r(\cdot), x(\cdot), u(\cdot)$, $y(\cdot), \dis(\cdot))$ that satisfies the system equations. We use the usual Lipschitz assumptions about the function $f$ so as to guarantee the existence and uniqueness of the solution. We introduce the notion of ``control setting'' to refer to a pair $s= (x_0, r(\cdot),\dis(\cdot))$ where $x_0$ is the initial state of the plant, $r(\cdot)$ is the reference signal, and $\dis(\cdot)$ is the disturbance signal. Let $\mathcal{S}$ denote the set of all possible control settings. Under each control setting $s$, the controller (represented by the function $f_c$) generates a behaviour, and for convenience we denote it by $\traj_s$. %For example, $x_0=(p(0), v(0))$ where $p(0)$ and $v(0)$ are the initial position and speed of a robot; $(p, v)$ may be only partial state of the plant. \myworries{examples of reference signals}
 
% We assume that we have a method of designing a nominal controller $C$ for the plant in some set $S$ of control settings, that is, for every $s=(x_0, r(\cdot)) \in S$ this controller can make the output $y$ of the plant, starting at the initial condition $x_0$ under the reference input signal $r(\cdot)$), track the reference $r$ while satisfying a property $\phi$ (specified by a temporal logic for example). The property $\phi$ can be, for example, reaching a goal point while satisfying some transient response specifications. As we shall see, the validity of this control design assumption will also be checked during our design process. 

\subsection{Control Specifications}
Our control objective is to make the output $y$ of the plant, starting at an initial condition $x_0 \in X_0$, track the reference $r$ while satisfying a property $\phi$ specified using STL. Before recalling STL, we remark that our framework deals with finite-time traces which cannot be used to prove liveness and stability properties. However, practical stability, such as convergence to a region (for example a neighbourhood of the origin) during a given time interval~\cite{Lasalle61}, has been intensively studied in theory and proven useful in practice. Furthermore, combining with invariant computation, finite-time traces can be used to falsify liveness properties (such as by showing the system will get trapped in some set after some finite time~\cite{Navarro-LopezC16}). STL and temporal logics in general have been used by the control community to specify various control performance properties~\cite{AMT20_2018}. Some examples of typical control specifications expressed in STL can be found in Sect.\;\ref{sec:experiment}.

\input{stl.tex} 

\subsection{Problem Definition}

Our goal is to generate a NN feedback controller so that the closed-loop system satisfies some desired properties, where the learning guidance is provided using positive examples, that is good behaviours. This learning-based approach is of particular interest when good behaviours cannot be generated by a single control law but only by combining different control laws. Indeed, when the plant is nonlinear, it is hard to find one controller of a fixed structure (such as PID, MPC) that performs well for all control settings, and it is 
time-consuming to fine-tune the parameters to adapt to new scenarios. Here we can see the interest of using NN controllers as a means of combining controllers. Indeed, by exploiting the approximation power of NN, they can be trained to achieve the qualities that are difficult to achieve jointly using conventional control methods. 

The problem addressed in this paper is formally presented below.

\begin{problem}[Learning of Feedback Controller]
Given a plant $\Pi$, a set of nominal controllers $\mathcal{C}$ and a set of STL specifications $\Phi$, learn a neural network controller $N$ with the help of the nominal controllers so that the closed-loop system with  plant $\Pi$ and controller $N$ satisfies all the specifications in $\Phi$.
\end{problem}

%\subsection{Nominal Controllers}
%We assume that we are given a nominal controller $C$ that can produce a desired closed-loop behaviour (satisfying the control specification) for every control setting $s=(x_0, r(\cdot)) \in S$. 
%In the remainder of the paper, let $C$ denote a nominal controller designed for every control setting $s=(x_0, r(\cdot)) \in S$. 
In the learning context, a nominal controller plays the role of a teacher that generates a desired closed-loop behaviour for a given control setting which the NN should learn. To do so, the nominal controller makes use of a collection of conventional controllers, each of which is responsible for a subset of control settings or satisfies a subset of desired control properties. In this paper we mostly focus on the problem of how to iteratively train NN using examples (good behaviours) and counterexamples (bad behaviours). A method for generating good behaviours combining different properties from a collection of controllers is illustrated via an example described in Sect.\;\ref{sec:experiment}.

==> iccps2023_version/property.tex <==
\begin{property}\label{property:matching} 
\textbf{Matching Error:} The closed-loop output of the plant, using the nominal controller $y$ and that using the NN controller $\overline{y}$ do not differ by more than $e$: 
%\is{Use either $y_{nn}$ or $\overline{y}$.}
$\Box_{[0,\simtime]} (|\overline{y}[t]-y[t]|< e)$.
%\end{mycenter}
%\[\Box_{[0,\simtime]} (|\overline{y}[t]-y[t]|< e)\]
%alw_[0,\simtime] (abs(\overline{y}[t]-y[t])<0.2)
%alw_[0,\simtime] (abs(\overline{y}[t]-y[t])<0.2)
\end{property}
\begin{property}\label{property:stabilization}
\textbf{Stabilization:} Whenever there is a step change of more than $\varepsilon_r$ in the reference $r$, then after time $T_1$ and within time $T_2$, the plant output $\overline{y}$ (under the NN controller) remains within $r \pm e$ for time $T_3$ to time $T_4$:~~ %\myworries{dt here???} 
%\begin{mycenter}[1pt]
$\Box_{[0,\simtime]}((|r[t+dt]-r[t]|>\varepsilon_r) \Rightarrow (\Diamond_{[T_1,T_2]} \Box_{[T_3,T_4]} (|\overline{y}[t] - r[t]|< e)))$.
%\end{mycenter}
%\[\Box_{[0,T_1]}((|r[t+dt]-r[t]|>d \vee [t]==0) \Rightarrow (\Diamond_{[0,T_1]} \Box_{[0,T_2]} |y_{nn}[t] - r[t]|< e)) \]
%alw_[0,\simtime]
%(
%   (abs(r[t+dt]-r[t])>d or [t]==0) => 
%   (
%        ev_[0,T_1] alw_[0,T_2] (abs(y_nn[t]-r[t])<e)
%   )
%)
\end{property}

\begin{property}\label{property:settling}
\textbf{Settling time: } Whenever there is an increasing (or a decreasing) step change in the reference $r$, the plant output $\overline{y}$ should settle to $r \pm e'$ within time $T_5$, and stay settled up to time $T_6$:
%$((r[t] > 10) \Rightarrow (\Box_{[1,3]}(y_{nn}[t]-r[t]<ov))) \wedge$ 
%$((r[t] \leq 10) \Rightarrow (\Box_{[1,3]}(r[t]-y_{nn}[t]<ov))) \wedge$
%\begin{mycenter}[1pt]
$(\Box_{[0,T_{sim}]} (|(r[t+dt]-r[t]| > \varepsilon_r) \Rightarrow (\Box_{[T_5,T_6]}(|\overline{y}[t]-r[t]|< e'))))$.
%\end{mycenter}


%((r[t] > 10) => (alw_[1,3](y_nn[t]-r[t]<ov))) and 
%((r[t] <= 10) => (alw_[1,3](r[t]-y_nn[t]<ov))) and 
%(alw_[0,sim_time] ((r[t+dt]-r[t] > d) => (alw_[1,3](y_nn[t]-r[t]<ov)))) and
%(alw_[0,sim_time] ((r[t]-r[t+dt] > d) => (alw_[1,3](r[t]-y_nn[t]<ov))))
\end{property}


\begin{property}\label{property:overshoot}
\textbf{Overshoot: }Whenever there is an increasing step change in the reference $r$, the plant output $\overline{y}$ should be at most $r+\ov$ for time $T_7$ to $T_8$ in the future: %\ih{1. For overshoot should it be greater and for undershoot it should be lesser? It should be then `greater (or lesser)' 2. $y_{nn}$ should be $ov$ lesser (or greater) than $r$ means that $y_{nn}-r[t]=\ov$ (or $r[t] - y_{nn} =\ov$)}
%\ih{Should we say `(or Undershoot)' also?} 
%$((r[t] > 10) \Rightarrow (\Box_{[1,3]}(y_{nn}[t]-r[t]<\ov))) \wedge$
%$((r[t] \leq 10) \Rightarrow (\Box_{[1,3]}(r[t]-y_{nn}[t]<\ov))) \wedge$
%\begin{mycenter}[1pt]
$\Box_{[0,\simtime]} ((|r[t+dt]-r[t]| > \varepsilon_r) \Rightarrow (\Box_{[T_7,T_8]}(\overline{y}[t]-r[t]<\ov)))$. % \wedge$
%$(\Box_{[0,\simtime]} ((r[t]-r[t+dt] > d) \Rightarrow (\Box_{[1,3]}(r[t]-y_{nn}[t]<\ov))))$
%\end{mycenter}


%((r[t] > 10) => (alw_[1,3](y_nn[t]-r[t]<ov))) and 
%((r[t] <= 10) => (alw_[1,3](r[t]-y_nn[t]<ov))) and 
%(alw_[0,sim_time] ((r[t+dt]-r[t] > d) => (alw_[1,3](y_nn[t]-r[t]<ov)))) and
%(alw_[0,sim_time] ((r[t]-r[t+dt] > d) => (alw_[1,3](r[t]-y_nn[t]<\ov))))
\end{property}


%\is{Property 2 and property 4 seem to have the same meaning. In fact property 4 seems to be redundant or even wrong when compared to Property 3.}

==> iccps2023_version/related.tex <==
\section{Related Work}
\label{sebsec-related}

Recent research has shown the feasibility of using deep neural networks as feedback controllers for nonlinear dynamical systems through supervised learning~\cite{Nicol08,LiQZBHS17,NIPS2017_7233,Chen18,sanchez2018real,varshney2019deepcontrol} and reinforcement learning~\cite{LillicrapHPHETS15,ZhangKLA16,hwangbo2017control,ChowNDG18}. 
However, for the neural network-based controllers to receive wide acceptability as an alternative of the traditional controllers like PID~\cite{visioli2006}, LQR~\cite{astrom2010feedback}, and MPC~\cite{mpc}, one should be able to establish safety and performance guarantees on the closed-loop system.
In the last decade, there has been significant progress in verifying neural networks against safety~\cite{huang2017safety,katz2017reluplex,Ehlers17,LomuscioM17,WangPWYJ18,Wenjie18,XiangTJ18,DuttaJST18A,IvanovCWAPL20} and robustness properties~\cite{ChengNR17,singh2018fast,RaghunathanSL18,GehrMDTCV18,TjengXT19,abs-1903-01287}.  These tools can bound the output set by tracking the evolution of the input set throughout the network and are useful in evaluating the soundness of a neural network in various vision applications. While such set propagation provides guarantees on safety and robustness properties specified for neural networks, such guarantees  are not sufficient for proving properties of the closed-loop system with a neural network acting as a feedback controller, since the soundness of the closed-loop system depends on dynamical interaction between the controller with the plant. Recently researchers have developed tools to address the verification problem for the closed-loop control systems~\cite{DuttaJST18B,ivanov2019verisig,dutta2019reachability,HuangFLC019}. 
These verification tools involve the reachability analysis of a hybrid system~\cite{frehse2011spaceex,ChenAS13,althoff2015introduction}, which is computationally hard, resulting in the tools to be not scalable.
Several research groups have developed methodologies for systematic testing of a closed-loop system with a neural network controller~\cite{ZutshiJ15,TianPJR18,YaghoubiF19,DreossiDS19,tran2020cav_tool,tran2020}. Though these methods are effective in identifying scenarios that detect the weakness of the neural network controller, counterexamples provided by reachability-based tools are often too abstract to enable accurate information for correcting the neural network controller.  

%{\color{red} REVIEW: Comparisons with existing methods. In particular, evidence should be presented for the claim that the existing methods of reachability analysis on closed-loop systems do not scale (line 82). => {\bf to GIVE SCALABILITY OF THESE TOOLS, TO check if we cited NNV and the latest}

%The benefit over [51] also requires more evidence. DONE

%"NN does not satisfy given requirements, reachability analysis tools do not provide feedback for correcting the NN." - Most of the verification approaches are model producing, that is, they generate counterexamples. So, aren't these counterexamples useful feedback for correcting the NN? DONE
%}

To avoid the complexity of verification of the closed-loop system with a neural network feedback controller, a number of recent papers have explored the possibility of synthesizing the correct-by-construction AI-based feedback controller.
Ferlez and Shoukry~\cite{FerlezS20} present a method for deciding the structure of the neural network controller with a guarantee that there exist the weights of the neural network that allow it to approximate an MPC precisely.
% As an alternative of neural network, Gaussian process has also been used to synthesized feedback controller with stability guarantee~\cite{NIPS2019_8355}.
Berkenkamp et at.~\cite{berkenkamp-nips17} demonstrated how a deep reinforcement learning algorithm can be applied to learn a neural network control policy without violating the safety requirements.
In~\cite{althoffRL}, a Reinforcement Learning method that uses temporal-logic falsification for adversarial learning is proposed. Instead of constructing a reward function for the adversary, they use falsification of metric temporal logic specifications. This work focuses on unsupervised learning unlike ours which is primarily tailored to supervised learning.

The principle of learning to control through counterexamples goes back to at least Henzinger et al.~\cite{henzinger2003counterexample}, who applied it to automata.
Chang et al.~\cite{ChangRG19} propose a methodology for the co-synthesis of NNs representing a feedback controller and a Lyapunov function certifying the stability of the closed-loop system. Their method relies on the refinement of the NNs based on the training data generated from the counterexample showing that the trajectory of the closed-loop system is violating the Lyapunov condition.  
The closest to our work is the paper by Clavi{\`{e}}re et al.~\cite{ClaviereDS19}, where the authors approximate the behavior of a model predictive controller with a deep neural network to enable a robot to follow a reference trajectory closely. They employ counterexample-guided refinement of the NN by generating additional training data from counterexamples. However, unlike our framework,  
their approach is limited to memoryless controllers, and they use tracking closeness as the sole criterion to identify counterexamples. 
In our experience, a NN need not always closely track the nominal behaviour to satisfy the specifications. It may have some characteristics that are better than the nominal controller, such as a smaller overshoot, or quicker stabilization in some areas of the state space. Such behaviours would be eliminated using their approach.

% In~\cite{ClaviereDS19}, the authors present a counterexample guided training of neural networks for the task of robustly tracking trajectories of robotic vehicles. Our work differs from theirs because we use Signal Temporal Logic (STL) specifications for falsification rather than random sampling and gradient descent. STL specifications have the advantage of being able to express more features than simple trajectory tracking. Our controller design also includes delay blocks while theirs is a simple feed-forward neural network.
Counterexample-guided retraining of neural networks for vision-based control has been attempted in a few recent work.
 In~\cite{seshiaVerifai}, a neural network is used to estimate the position of an aircraft from a camera image. A controller then keeps the plane close to the center-line of the runway. Finally, falsification and debugging are used to retrain the neural network and make the closed-loop system robust. In~\cite{cexRavan}, the authors present a framework that iteratively build simple surrogate models of complex perception modules. The framework uses a falsifier to find counterexamples, that violate a safety property to extract information that lets us obtain efficient modelling of perception modules and errors in it. Counter Example Guided Inductive Synthesis (CEGIS) is used to synthesize controllers that satisfy the given specifications. If the obtained policy is not safe, we use the counterexamples and repeat the process until a controller is found that can keep the system safe despite perception failure. 
 %However, in contrast to our work, the controllers used in~\cite{seshiaVerifai,cexRavan} are not based on neural networks.
% In our experience, a NN may not always closely track the nominal behaviour, but can have some characteristics that are better than the nominal, such as a smaller overshoot, or quicker stabilization in some areas of the state space. Such behaviours would be eliminated using their approach.
% \ab{However, unlike our framework, they use tracking closeness as the sole criteria to identify counterexamples. In our experience, a NN may not always closely track the nominal behaviour, but can have some characteristics that are better than the nominal, such as a smaller overshoot, or quicker stabilization in some areas of the state space. Such behaviours would be eliminated using their approach.}

%\myworries{Add organization}

==> iccps2023_version/removed.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% This file contains text that was removed from the draft
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\subsection{Motivation}
\paragraph{Problem Definition}
We consider a plant with state $x \in \mathbb{R}^n$
\begin{eqnarray}
x_{k+1} &= &f(x_k,u_k),\\
y_k &= &h(x_k) 
\end{eqnarray}
and inputs $u_k\in \mathbb{R}^p$ and measurable outputs $y_k\in \mathbb{R}^q$.
We have a \emph{nominal} controller with state(!)
\begin{eqnarray}
z_{k+1} &= &f_c(z_k,y_k,w_k), \\
u_k &= &g(z_k,y_k,w_k)
\end{eqnarray}
that for all values of the reference signal $w$ leads to state trajectories that satisfy a given closed-loop specification
$$\forall w(\cdot),x_0: x(\cdot) \in \mathbb{S}(w(\cdot)).$$
For example, we desire that when $w$ changes from one constant value to another (step response), $y$ is close to the reference $w$ within some time frame, with an overshoot that does not exceed a certain threshold.
%
For reasons beyond the scope of this document, we wish to replace the nominal controller with a neural net (NN) controller. We assume a nonlinear autoregressive (ARX) structure that uses the past $T$ measurements, reference values, and control actions:
$$\hat u_{k+1} = \hat c(y_k,w_k,u_k,\ldots,y_{k-T},w_{k-T},u_{k-T}).$$
%

%
In this paper, we address the problem of how to train the NN controller such that it satisfies the closed-loop specification.
%
For our purposes, a NN is simply a function
$$b = N_T(a),$$
which is constructed from a training set of $n_T$ values $$T = \{(a_1,b_1),\ldots,(a_{n_T},b_{n_T})\}.$$
%
The outcome of training our net is not known a priori. In particular, we do not assume that the training data is learned perfectly, which means that in general $N_T(a_i) \neq b_i$.
%
To assess the trained net, we look at its response to a set of stimuli from a \emph{test set} $$R = \{(\hat a_1,\hat b_1),\ldots,(\hat a_{n_T},\hat b_{n_T})\}.$$ 
%
We evaluate the performance of the net on the training set with a \emph{test metric} $d_R$ that compares the output $N_T(\hat a_i)$ to the nominal value $\hat b_i$. We say that the net \emph{satisfies the test metric} if for all $a_i \in R$, $$d_R(N_T(a_i),b_i)\leq 1.$$
\is{What is the significance of the value ``1''?}
%
Note that the training and test sets may be constructed iteratively, alternating phases of training and testing.
%
We can characterize our \emph{sound training problem} as follows.
%
\textinbox{
Given a nominal controller, a plant, and an untrained neural net $N$, find a training set $T$, a test set $R$, and a test metric $d_R$ such that if the trained net satisfies the test metric, then for all reference signals, the state trajectories satisfy the closed-loop specification.
}

Ideally, we would like our training procedure to be complete in the following sense (maybe for linear systems this can be achieved):
%
\textinbox{
Given a nominal controller and a plant, construct a sequence of neural nets $N_i$,  training sets $T_i$ and test sets $R_i$ such eventually (for some $i$) the sound training problem is solved.
}


\paragraph{Closed-Loop vs Open-Loop Training}
%
%
In principle, our task is to approximate the (stateful) control function with the ARX function $\hat f_c$. We discuss some of the difficulties that make it attractive to train the NN controller in closed-loop rather than open-loop.

\paragraph{Unknown ARX horizon}
The first problem is that our nominal controller is not in ARX form.
Assume wlog. that $z_0=0$.
Then we can rewrite the nominal controller to an ARX equation of length $k$:
\begin{eqnarray}
u_k &= &g(f_c(z_{k-1},y_{k-1},w_{k-1}),y_k,w_k) \\
 &= &g(f_c(\ldots(f_c(z_{0},y_{0},w_{0})\ldots),y_{k-1},w_{k-1}),y_k,w_k)\\
 &=: &c(y_k,w_k,u_k,\ldots,y_{0},w_{0},u_{0})
\end{eqnarray}
%
From the above equation it is clear that we try to approximate an ARX equation of growing length with one of fixed length $T$.
\highlight{Without considering the plant, it may be difficult to decide  how short the ARX horizon $T$ can be without degrading performance.}

\paragraph{Explosion in the Number of Training Samples}
%
Assume our nominal controller is also ARX of length $T$.
So our goal is to approximate the nominal control function
$$c(y_k,w_k,u_k,\ldots,y_{k-T},w_{k-T},u_{k-T})$$
with the NN function
$$\hat  c(y_k,w_k,u_k,\ldots,y_{k-T},w_{k-T},u_{k-T}).$$
%
Consider doing this in open-loop training.
We could regularly sample the domain of $y,w,u$ with a grid, and train $\hat c$ on those grid points.
Assume the grid covers each variable with $N$ values and that $y,w,u$ are $d$-dimensional vectors. Then there are $N^{3dT}$ 
points in the grid. 
\highlight{Learning based on a uniform distribution is exponential in the signal dimension and the ARX horizon. For even modest values of $N$ and $T$, this becomes prohibitively large.
In contrast, the closed-loop system only traverses a limited subspace. For a fixed reference $w$, it amounts roughly to sampling a single trajectory. Closed-loop learning largely depends on the space of considered reference trajectories, not the control or state space (assuming a small set of initial states).
}

\paragraph{Required Sample Density Unknown}
%
It is by no means clear that a uniform distribution of training samples
is an efficient way to learn the controller.
\highlight{In some of our experiments, we removed points that we considered redundant. This lead to a drastic drop in learning performance.
On the other hand, using all the samples from closed-loop operation lead to good performance, despite seeming redundant.
}

\paragraph{Approximation Distance does not Imply Performance}
%
Conventional function approximation would learn $\hat c$ such that $\hat c$ and $c$ are close according to some metric.
When standard metrics (Euclidian) are used, this does not automatically imply good performance with respect to a behavioral metric.
\highlight{Some of our experiments suggest that large deviations in control output can be tolerated during transitions, while good steady-state behavior requires high accuracy around the operating point.}



==> iccps2023_version/stl.tex <==
An STL formula $\spec$ consists of atomic predicates along with logical and temporal connectives. Atomic predicates are defined over signal values and have the form $g(\outsig(t))\sim 0$, where $g$ is a scalar-valued function over the signal $\outsig$ evaluated at time $t$, and $\sim \in \{ <,\leq, >, \geq, =, \neq \}$. 
Temporal operators ``always'' ($\globally$), ``eventually'' ($\F$), and ``until'' ($\until$) have the usual meaning 
%\is{We may need to provide more intuitive details about the temporal operators. The audience in this conference may not be familiar with temporal logic and may complain that our paper is not fit for the conference.}
and are scoped using intervals of the form $(a,b)$, $(a,b]$, $[a,b)$, $[a,b]$, or $(a,\infty)$, where 
$a,b\in \reals_{\geq 0}$ and $a<b$. If $I$ is a time interval, the following grammar defines the STL language.
\begin{equation}~\label{eqn:stl-gen}
\spec ~ := ~ \true \; | \; g(\outsig(t))\sim 0 \; | \; \neg \spec \; | \;
\spec_1 \wedge \spec_2 \; | \; \spec_1 \until_I \spec_2:~~\sim \in \{ <,\leq,>,\geq,=,\neq \}
\end{equation}
The $\F$ operator is formally defined as $\F_I \spec \triangleq \true \until_I \spec$, and the $\globally$ operator is defined as $\globally_I \spec \triangleq \neg (\F _I \neg \spec)$. When omitted, the interval $I$ is taken  to be $[0,\infty)$. 
%\ih{Do we need to define $\U_I$?} 
%\is{Equivalence symbol is not being printed on the paper.}
%The semantics are described informally as follows.
%The signal $\outsig$ satisfies $f(\outsig)> 0$ at time $t$ if $f(\outsig(t))>0$. It satisfies $\spec = %\G_{(0,1]}(f(\outsig)=0)$ if for all time $0< t \leq 1$, $f(\outsig(t))=0$. The signal satisfies $\spec= %\F_{[1,2)}(f(\outsig)<0)$ iff there exists a time $t$ such that $1\leq t < 2$ and $f(\outsig(t))<0$. %The %two-dimensional signal $\outsig=(\outsig_1,\outsig_2)$ satisfies the formula %$\spec=(\outsig_1>0)\U_{[2.8,4.5]}(\outsig_2<0)$ iff there is some time $t$ where $2.8 \leq t \leq 4.5$, %$\outsig_2(t)<0$, and $\forall t'$ in $[2.8,t)$, $\outsig_1(t')>0$.
%\myworries{define Until with interval}
 The ``always'' operator in $\globally\spec$ conveys that from the current time point onwards, $\varphi$ always holds. The ``eventually'' operator in $\F\spec$ means that there exists a time point in the future where $\spec$ holds. The ``until'' operator in $\spec_1\until\spec_2$ means that, starting from the current time point $\spec_1$ should hold continuously until a future time point where $\spec_2$ holds. Additionally, an interval $I$ can be combined with the operators to bound their scope to a segment of time in the future rather than the whole. For example, $\spec_1\until_{[a,b]}\spec_2$ holds true at time $t$ if $\spec_2$ holds true at some point $t'\in[t+a,t+b]$ and $\spec_1$ is always true in $[t,t']$. 
 
 Given a signal $\outsig$ and an STL formula $\spec$, we use the quantitative semantics for STL, which 
is defined formally in~\cite{DonzeM10}. %\ih{DonzeM10 is not added to any of the bibtex files.}
%\is{The command outsig is not being printed.}
The quantitative semantics defines a function $\rho$ such that when $\rho(\spec,\outsig,t)$ is positive it indicates that $(\outsig,t)$ satisfies
$\spec$, and its absolute value estimates the \emph{robustness} of
this satisfaction. If $\spec$ is an inequality of the form
$g(\outsig)>b$, then its robustness is $\rho(\spec,\outsig,t) = g(\outsig(t))-b$.  
When $t$ is omitted, we assume $t=0$ (i.e., $\rho(\spec,\outsig)=\rho(\spec,\outsig,0)$ ). For the conjunction of two formulas $\spec := \spec_1 \wedge \spec_2$, we have
$\rho(\spec,\outsig)=\min \left( \rho(\spec_1,\outsig),\rho(\spec_2,\outsig)\right)$,
while for the disjunction $\spec := \spec_1 \vee \spec_2$, we have
$\rho(\spec,\outsig)=\max\left(\rho(\spec_1,\outsig),\rho(\spec_2,\outsig)\right)$. For negation, $\rho(\neg\spec,\outsig)=-\rho(\spec,\outsig)$.
%\is{What about negation?} 
For a formula with until operator as $\spec := \spec_1 \until_I \spec_2$,
the robustness is computed as:\\ $\rho(\spec,\outsig,t) = \max_{t^\prime\in
  I}\left(\min\left(\rho(\spec_2,\outsig,t^\prime),\min_{t^{\prime\prime}\in
  [t,t^\prime]}\left(\rho(\spec_1,\outsig,t^{\prime\prime})\right)\right)\right).$  %{\color{red} Thao: I changed f to g in predicates as suggested by a reviewer, please double check if I miss any }
  


